Coloring a Dominating Set Without Conflicts: q-Subset Square Coloring

The \emph{Square Colouring} of a graph $G$ refers to colouring of vertices of a graph such that any two distinct vertices which are at distance at most two receive different colours. In this paper, we initiate the study of a related colouring problem called the \emph{subset square colouring} of graphs. Broadly, the subset square colouring of a graph studies the square colouring of a dominating set of a graph using $q$ colours. Here, the aim is to optimize the number of colours used. This also generalizes the well-studied Efficient Dominating Set problem. We show that the q-Subset Square Colouring problem is NP-hard for all values of $q$ even on bipartite graphs and chordal graphs. We further study the parameterized complexity of this problem when parameterized by a number of structural parameters. We further show bounds on the number of colours needed to subset square colour some graph classes.

==> BP.tex <==

A graph is a bipartite permutation graph if it is both bipartite and permutation graph. Bipartite permutation graphs. 
Let $G(A\cplus B, E)$ be a bipartite permutation graph, where $A$ and $B$ are independent sets and it admit strong ordering, adjacency and enclosure properties.

\begin{definition}
An ordering of the vertices $A$ in a bipartite graph $G(A\cplus B, E)$ has the adjacency property if for each vertex $v \in B$, $N(v)$ are consecutive in the ordering of $A$.
\end{definition}
\begin{definition}
An ordering of the vertices $A$ in a bipartite graph $G(A\cplus B, E)$ has the enclosure property if for every pair of vertices $v, u \in B$ such that $N(v)$ is a subset of $N(u)$, vertices in $N(u)-N(v)$ occur consecutively in the ordering of $A$. 
\end{definition}

\begin{definition}
A strong ordering of the vertices of a bipartite graph $G(A\cplus B, E)$ consists of an ordering of $A$ and an ordering of $B$ such that for all $(a, b')$, $(a', b)$ in $E$, where $a, a'$ are in $A$ and $b, b'$ are in $B$, $a < a'$ and $b < b'$ imply $(a, b)$ and $(a', b')$ are in $E$. 
\end{definition}

%In this 3-tuple $G = (A, B, E)$, every edge in $E$ connects a vertex in $A$ and another vertex in $B$. Vertices of $A \cup B$ are
numbered  in  the  permutation  ordering. Let  $A = \{a_1, a_2, \cdots a_n\}$ and $B = \{b_1, b_2, \cdots b_m\}$, where  $A$ and $B$ are in the strong ordering such that $a_i < a_i'$ iff $1 \leq i < i'\leq n$ and $b_j < b_j'$, iff $1 \leq j < j' \leq m$, respectively. Let $s(v) = \min N(v)$ and $l(v)= \max N(v) $ be the smallest and largest vertex adjacent to $v$ respectively.
	Now we give a dynamic programming algorithm to solve the \SH problem for this instance.
	 W.l.o.g lets consider $b_{i,j}$ be the vertex in $a_i \in A$ that dominate the vertex in $b_j \in B $ and $c$ be minimum number of conflict free colors used so far.
	
	Let $dp[i, j, c]$ returns the minimum number of conflict free colors used till $b_j \in B$. Thus the desired solution is returned by $dp[i>0,1, c\leq 2 ]$. We now give a recurrence relation to compute $dp[i, j]$.
	
	

	\begin{equation}
	dp[i,j,c]_{1 \leq j \leq m}= \min c_{  i' > i \in A and 1 \leq i' \leq n, where j \in N[i']} \big\{ dp[i', j, c \}
	\end{equation}
	
To see the correctness of the above, observe that the recurrence considers  all $j$ which is dominated by $i$. For the correct guess of $a_i$,cover all $N[a_i]$ including $j$. In the remaining solution of $a_i'$ if $N[a_i'] \cap N[a_i = \phi$, then we can reuse the color of $a_i$. Similarly for an uncovered vertices in $B$, similar $dp[j, i, c]$ will work. If we combine the $dp[i, j, c]$ and $dp[j, i, c]$ use only at most four colors. 

	It is clear that computing the value of one DP table entry takes $O(m)$ time. The number of $dp[ *, *]$ values to be computed is clearly $O(n^2)$ time.  Therefore, the algorithm runs in $O((nm)^2)$ time.
	



==> BPP3.tex <==
\vspace{.1cm} 
 \noindent In this section we discuss bounds on $\chi_{ssc}$ for bipartite permutation graphs.\\
A graph is a bipartite permutation graph if it is both bipartite and permutation graph. Let $G(A\uplus B, E)$ be a connected bipartite permutation graph, then it admits the strong ordering, adjacency and enclosure properties, as defined below~\cite{BPg}.
\begin{enumerate}
\item An ordering of the vertices $A$ in a bipartite graph $G(A\uplus B, E)$ has the \emph{adjacency property} if for each vertex $v \in B$, the vertices in $N(v)$ are consecutive in the ordering of $A$.
\item An ordering of the vertices $A$ in a bipartite graph $G(A\uplus B, E)$ has the \emph{enclosure property} if for every pair of vertices $v, u \in B$ such that $N(v)$ is a subset of $N(u)$, vertices in $N(u)-N(v)$ occur consecutively in the ordering of $A$. 
\item \emph{A strong ordering} of the vertices of a bipartite graph $G(A\uplus B, E)$ consists of an ordering of $A$ and an ordering of $B$ such that for all $(a, b')$, $(a', b)$ in $E$, where $a, a'$ are in $A$ and $b, b'$ are in $B$, $a < a'$ and $b < b'$ imply $(a, b)$ and $(a', b')$ are in $E$. 
\end{enumerate}
\begin{lemma}
If $G$ is a connected bipartite permutation graph, then $\chi_{ssc}(G) \leq 3$.
\end{lemma}
Let  $A = \{a_1, a_2, \cdots a_n\}$ and $B = \{b_1, b_2, \cdots b_m\}$ have the strong ordering property. For $a_j\in A$, let $s(a_j) = \min\{i|b_i \in N(a_j)\}$ and $l(a_j) = \max\{i|b_i \in N(a_j)\}$ be the smallest and largest vertex adjacent to $a_j$ respectively. (Symmetrically defined for $B$).

Now we colour a subset of vertices from $A$ and $B$, such that all vertices in $G$ are dominated. We can find an augmenting path in $G$ such that the vertices are in lexicographical order.
In the first step, we find the first two vertices of the augmenting path. The first vertex $v \in \{a_1,b_1\}$ such that $s(v)$ is the smallest vertex.% i.e, if $a_i$ is the first vertex, then $s(a_1) < s( b_1)$.
Without loss of generality, assume that $s(a_1)$ is the smallest vertex, then we colour $a_1$ using colour one and $s(a_1)$ using colour two. 
Let's assume $b_{j'} =s(a_1)$ in $B$. The third vertex in the path is $a_{i'} \in A$ such that $i'$ is the largest integer such that $N(b_{j'})$ contains $a_{i'}$. Colour it using colour three.  
 
In the $k^{th}$ step, we consider the smallest $j$ such that $b_j \in B$ and $b_j$ contains in $N(a_i)$, where $a_i$ is the vertex in the path added in $k-1^{th}$ step. Colour $b_j$ using a colour which is not been used so far.
%. Then we colour $a_i \in A$ such that $i$ is the largest integer such that $N(a_i)$ contains $b_j$, using colour one, if $k$ is odd, or otherwise, using colour two.
Repeat this till every vertex in $G$ is dominated. Now, if $a_i, a_j, a_k \in A$ are coloured in consecutive steps, then $N(a_i)$ and $N(a_k)$ are disjoint. 
For contradiction, assume that $N(a_i) \cap N(a_k) \neq \emptyset$. Let $j'=l(a_i)$. Then the vertex $b_{j'+1}$ is dominated by both $a_j$ and $a_k$. This contradicts that $a_j$ was coloured by the algorithm to dominate $b_{j'+1}$. Thus no vertex in $A$ or $B$ has repeating colours in its neighbourhood. This proves the result. \qed
\vspace{.1cm}


==> Distance_to_Cluster.tex <==

\subsection{The \SH parameterized by distance to cluster graph}



\begin{definition}
A cluster graph is a disjoint union of complete graphs.
\end{definition}
It is easy to see that cluster graphs can be $1$-subset square colored.
%\begin{definition}
%A cluster vertex deletion set $X$ of a graph $G$ is a set of vertices such that $G\backslash X$ forms a cluster graph.
%\end{definition}
%\noindent
%The cluster vertex deletion number is defined as the minimum possible size of cluster vertex deletion set $X$. Intuitively, it is the measure of how close a graph is to being a cluster graph.
 In this section, let $X \subseteq V(G)$ such that $G[V\setminus X]$ is a cluster graph and $|X| =k$. Now we observe the connection between $\chi_{ssc}(G)$ and $k$.

\begin{lemma}\label{sharCVDSbound}
 $\chi_{ssc}(G)\leq |X|+1$.
\end{lemma}

\begin{proof}
To subset square color graph $G$, we color each vertex $v \in X$. If the size of $X$ is $k$, then we have utilized $k$ colours. Now color exactly one of the undominated vertices in each complete graph(s) in $G\backslash X$ using a color that is different from previously used $k$ colors. Note that two colored vertices $u$ and $v$ in two different cluster graphs do not have a common neighbor in $X$ because in such a scenario, we would not choose either of $u$ or $v$ to assign it the $(k+1)^{th}$ color. We assign $(k+1)^{th}$ color to an $undominated$ vertex in each cluster graph which implies that this vertex is not adjacent to any vertex in $X$. This gives us a \sh of $G$ as the vertices in $X$ are dominated by the colors assigned to them. Additionally, some of the vertices in $G\backslash X$ may also have a neighbor in $X$. Every $v \in V(G)$ has at least one colored neighbor in $N[v]$ and in case more than one colored vertices are present in $N[v]$, we are assured of them being distinct because we have used $k+1$ colors. Therefore the result follows.
\end{proof}


\begin{theorem}
The \SH is FPT when parameterized by distance to cluster graph.
\end{theorem}

\begin{proof}
If $q \geq |X|+1$, then by Lemma~\ref{sharCVDSbound} it is trivially true that a \sh exists. Therefore, we assume that $q <|X|+1$. 
Let $G(V,E)$ be the graph and $X \subset V$ be the set of vertices such that $G[V-X]$ is cluster graph. Let $|X| \leq k$.
Consider all possible $(q + 1)^k$ \sh of $X$ using colors $\{c_0,c_1,\dots,c_q\}$. Here coloring by $c_0$ corresponds to a vertex not being colored. We tries to extend the coloring to a valid subset square coloring using $q$ colors of $G$ as follows.

%Let $\chi$ be such a coloring of $X$ such that no vertex in $V$ has the same color repeated in its closed neighborhood. We say a coloring $\chi_G$ of $V$ \emph{extends} $\chi$ if  $\chi_G$ restricted to $X$ is $\chi$. Our algorithm tries to extend each of the colorings to a valid subset square coloring using $q$ colors of $G$ as follows.

A subset of vertices in $X$ may not be dominated due to absence of a colored vertex in its closed neighborhood, say $Z$. Therefore, we require to color the neighbor(s) of the vertices in $V-X$ i.e clique vertices. In each clique, retain one vertex and delete all other vertices which have no neighbors in $X$. If we color a retained vertex, it  can dominate all deleted vertices, since it is a clique.
Furthermore, vertices in $Z$ can only dominated by the vertices from $V-X$. 

Note that if two or more vertices in a clique have the same neighborhood in $X$, then we retain one such vertex in clique and delete others. Now one clique can have at most $2^k$ such vertices. 


To bound the number of cliques as follows,
Let order the vertices in $Z$, say $v_1, v_2, \dots v_k$. Each clique is assigned by a bit stream of size $2^k$ such that bit stream positions are defined by subset of vertices in $Z$.

If a vertex in a clique have neighbor(s), say $v_i$, $1\leq i \leq k$ in $Z$, then bit stream of that clique is defined as a binary string, where the string contain value $1$ in positions of the all subsets which contain $v_i$, otherwise $0$.
 %For every clique, bit stream is defined as, if a vertex have neighbor(s) in $Z$, then corresponding position in bit stream have value one otherwise zero. 
Now each clique have a bit stream, with respect to the edges between vertices in clique and $Z$ .
If two or more bit streams are equal then retain one clique with same bit stream and delete all other, because they are dominating the same set of vertices in $Z$. Now we will be left with the clique which have unique bit steams. Therefore we can bound number of cliques by $2^{2^{k}}$ since, total number of vertices in $V-X$ bounded by $2^{2^{k}}.2^k$. Hence we can color the vertices in $\mathcal{O}(k^{(2^{2^{k}}.2^k)})$ using brute force.

\end{proof}

 %Hence the running time of the algorithm is $\mathcal{O}(k^{k^2.2^k})$

==> Distance_to_Threshold.tex <==
\begin{definition}
\cite{golumbic} A graph is a threshold graph if it can constructed from the empty graph by repeatedly adding either an isolated vertex or a dominating vertex.
\end{definition}

\begin{lemma}\label{threshold}
If $G$ is a threshold graph then $\chi_{ssc}(G) = 1$.
\end{lemma}

\begin{proof}
If isolated vertices are present, colour them using the same colour. By colouring the last introduced dominating vertex $v$, we satisfy \sh colour $G$ as each vertex in $G$ has only one coloured vertex $v$ in its closed neighbourhood.
\end{proof}

\begin{theorem}
The \SH is FPT when parameterized by distance to threshold graph.
\end{theorem}
\begin{proof}
Let $G(V,E)$ be the graph and $S \subset V$ be the set of vertices such that $G[V-S]$ is threshold graph. If $|S| \leq q$, then from the lemma \ref{threshold} it is trivially true that a \sh exists. Therefore we assume that $q \leq |S|$.\\
Consider all possible ${q+1}^k$ colouring of $S$ using colors $\{c_0, c_1, c_2, \cdots c_q\}$. the color $c_0$ used for the vertices which is not being colored. Let $\chi$ be such a coloring of $X$ such that no vertex in $V$ has the same color repeated in its closed neighborhood. We say a coloring $\chi_G$ of $V$ \emph{extends} $\chi$ if  $\chi_G$ restricted to $X$ is $\chi$. Our algorithm tries to extend each of the colorings to a valid subset square coloring using $q$ colors of $G$ as follows.

Let $X \sqcup Y=V-S$ , where $X$ is a independent set and $ \exists v \in Y$ with $d(v)=|Y|-1$. Consider the vertex $v \in Y$ which is adjacent to the all other vertices in the set $Y$. We can dominate all vertices in $Y$, by coloring $v$ using single color. Otherwise we may need more that $q$ color to dominate all vertices in $Y$. 
Now we need to dominate the vertices in $X$ that are not dominated. Observe that $v \in S$ can have at most $q$ such neighbors in $X$, because each of them needs to be colored using a distinct color.

The number of vertices in $X$ is therefore bounded by $kq$ which is at most $k^2$ as $q \leq k$.  We can now color the vertices in $X$ in $\mathcal{O}(k^{k^2})$ using brute force.

\end{proof}

==> GraphClass.tex <==

\subsection{Bounds for \SH colouring with respect to some classes of graphs}



\begin{definition}
Consider a graph $G$ on $n$ vertices. A complete graph $K_n$ is a graph $G$ on $n$ vertices with an edge between any two vertices $u,v \in V(G)$.
\end{definition}

\noindent
Let us analyse the number of colours required to \SH colour a complete graph $K_n$.


\begin{lemma}\label{completeG}
If G is a complete graph on n vertices then $\chi_{S1H}(G) = 1$.
\end{lemma}

\begin{proof}
The graph $K_n$ has each vertex adjacent to every other $n - 1$ vertices in the graph. Therefore, by assigning a colour to any one vertex of the graph will ensure that each vertex $v \in K_n$ is adjacent to the vertex that is assigned a colour. So this gives us a \SH colouring of $K_n$ such that $\chi_{S1H}(G) = 1$.
\end{proof}
\begin{corollary}
If a graph $G$ with a vertex $v$ which has an edge between each vertex $u \in G$, then $\chi_{S1H}(G) = 1$. Examples of such graphs are wheel graph ,flower graph, double wheel graph,etc.
\end{corollary}


\begin{lemma}\label{pathG}
If $G$ is a path on n vertices then $\chi_{S1H}(G) = 1$.
\end{lemma}
\begin{proof}
Any path on $n$ vertices requires exactly one colour to be \SH coloured. We give a constructive proof of this. Consider a path $P_n$ such that it has $3k$ or $3k + 2$ vertices where $k \geq 1$. We can colour every third vertex beginning from the second vertex from one of the end vertices of the path. For path of length $3k+1$, we can colour the first vertex using colour 1 and every third vertex using the same colour and so on. This ensures that every vertex is dominated by exactly one coloured neighbour in its closed neighbourhood.
\end{proof}



\begin{lemma}
If G is a cycle on $3n$ vertices then $\chi_{S1H}(G) = 1$. Further, if G is a cycle on $3n + 1$ or $3n + 2$ vertices then $\chi_{S1H}(G) = 2$.
\end{lemma}
\begin{proof}
For a cycle on $3n$ vertices, we colour every third vertex and hence get a \SH colouring using 1 colour. For cycles on $3n+1$ and $3n+2$ vertices, we use colour 1 to colour every third vertex beginning from a vertex, say $v_1$, and finally use colour 2 to colour the last vertex that appears in this sequence. 


Furthermore, we note that one colour is not sufficient for cycles on $3n + 1$ or $3n + 2$ vertices. Consider a cycle on $3n+1$ vertices. To \SH colour this cycle using one colour, we start by colouring vertex $v_1$ and assign the same colour to every third vertex. We observe that the vertex $v_n$ is also assigned the same colour as $v_1$, which does not \SH colour vertices $v_1$ and $v_n$. Therefore, to avoid this conflict, we colour vertex $v_n$ using a new colour. Now consider a cycle on $3n+2$ vertices. We colour the vertices using one colour, as it was done for cycles on $3n+1$ vertices. We observe that vertices $v_1$ and $v_{n-1}$ of the cycle on $3n+2$ vertices are coloured using the same colour. So, to dominate vertex $v_n$, we assign it a new colour. Therefore, for cycles on $3n+1$ and $3n+2$ vertices, we have $\chi_{S1H}(G) = 2$.
\end{proof}



\begin{definition}
A graph is a lollipop graph if it consisting of a complete graph with $m$ vertices and a path $P_n$, where end vertex of path is attached to one of the vertex in the complete graph.
\end{definition}

\begin{lemma}
If G is a lollipop graph $(G)$ then $\chi_{S1H}(G) = 1$.
\end{lemma}

\begin{proof}
From the lemma \label{completeG}, chromatic number of complete graph is one. 
Consider a path $P_n$ which is connected to complete graph at vertex $v$, such that it has $3k + 2$, $3k + 1$ vertices where $k \geq 1$. We can colour the vertices on $P_n$, as same as proof given in the lemma \label{pathG}. Since first vertex in the $P_n$ is coloured, every vertex in the complete graph is dominated by the first vertex in $P_n$. 
If $P_n$ has $3k$ vertices where $k \geq 1$, then we can colour every third vertex beginning from the end vertices of the path. All the vertices in the complete graph and the first vertex in $P_n$ are dominated by any vertex other than $v$ from the complete graph. This ensures that every vertex is dominated by exactly one coloured neighbour in its closed neighbourhood.

\end{proof}



\noindent
Now we study the nature of \SH colouring with respect to threshold graphs.

\begin{definition}
\cite{golumbic} A graph is a threshold graph if it can constructed from the empty graph by repeatedly adding either an isolated vertex or a dominating vertex.
\end{definition}


\begin{lemma}
If G is a threshold graph then $\chi_{S1H}(G) = 1$.
\end{lemma}

\begin{proof}
If isolated vertices are present, colour them using the same colour. By colouring the last introduced dominating vertex $v$, we satisfy \SH colour $G$ as each vertex in $G$ has only one coloured vertex $v$ in its closed neighbourhood.
\end{proof}


 
\begin{definition}
A graph is a sunflower graph $SF_n$ is a graph obtained by adding triangle on  each edge of the rim of a wheel graph $W_n$, such that two triangles,say petals share a common vertex if and only if the corresponding edges in $W_n$ are adjacent in $W_n$.
\end{definition}


\begin{lemma}
If G is a sunflower graph on $n$ vertices, where $n=odd$ then $\chi_{S1H}(G) = 2$. Otherwise $\chi_{S1H}(G) = 3$.
\end{lemma}

\begin{proof}
If we colour the vertex $v$, which has an edge between all vertices on the outer cycle on the $W_n$, Then all vertices on $W_n$ will be dominated by $v$. Since two petals share a vertex, we need exactly two colours and we can alternatively use the colours to dominate all petals. Therefore we need three colours to dominate $SF_n$, where $n$ is even. If we dominate the vertex $v$ by a vertex $u$ from the outer cycle on the $W_n$, then two petals are dominated by $u$,which are share the vertex $u$. We need exactly two colours to dominate all petals. Since we can reuse the colour of $u$ for the petals where $u$ is not part of it. Therefore we need only two colours to dominate $SF_n$, where $n$ is odd. If we use the same way of subset-1-harmonious colouring of $SF_n$, where $n$ is even, to dominate the vertex $v$ by a vertex $u$ from the outer cycle on the $W_n$ in $SF_n$, where $n$ is even. Then also we need one more colour to dominate the petal, which is adjacent to a petal, where $u$ is part of it. Therefore any possible subset-1-harmonious colouring (either colour the vertex $v$ or $u$) of $SF_n$, where $n$ is even needed three colours.
\end{proof}

Now using the similar proof of \SH colouring with respect to sun graphs. Corollary follows, 

\begin{definition}
A graph is a sun graph $SF_n$ is a graph obtained by adding triangle on adjacent vertices of the outer cycle of the complete graph graph $K_n$, such that two triangles,say petals share a common vertex if and only if the corresponding edges in outer cycle of $K_n$ are adjacent in $K_n$.
\end{definition}

\begin{corollary}
\label{sun}
If G is a sun graph on $n$ vertices, where $n=odd$ then $\chi_{S1H}(G) = 2$. Otherwise $\chi_{S1H}(G) = 3$.
\end{corollary}


 






\begin{definition}
A graph is a grid graph if and only if it is an induced subgraph of a grid 
A two-dimensional grid graph ($m\times n$), also known as a rectangular grid, which is Cartesian product of $P_m$and $P_n$.

\end{definition}


\begin{lemma}
If G is a grid graph then $\chi_{S1H}(G) = 2$.
\end{lemma}

\begin{figure}[htb]
\centering
\includegraphics[scale=0.5]{Grid.pdf}
\caption{\SH colouring using two colour on grid graphs}
\label{Figure: grid}
\end{figure}

\begin{proof}
Any grid $1 \times 1$ needs exactly two vertices, shown in figure \ref{Figure: grid}(a). In general, $m \times n$ grid requires exactly two colours in \SH colouring. We give a constructive proof of this. Consider a $3 \times 3$ grid, which can be coloured using two colours shown in figure \ref{Figure: grid}(b). This ensures that every vertex is dominated by exactly one of the coloured neighbour in its closed neighbourhood. For $3k \times 3k$ grid, in every column we repeat the same colouring shown in \ref{Figure: grid}(b). In every row we alternatively use the colouring shown in \ref{Figure: grid}(b) and (c). From this colouring we can observe that paths in the $(3k+1)^{th}$ row and $(3k+1)^{th}$ column in $(3k+1) \times (3k+1)$ grid are self dominated by one colour, shown in figure \ref{Figure: grid}(d). Therefore to dominate paths in the $(3k+2)^{th}$ row and $(3k+2)^{th}$column can also be dominated using two colours.

\end{proof}


\begin{definition}
A graph is a grid caterpillar graph if and only if it is a tree having a chordless
path $P_t$ on t vertices, called central path, which contains atleast one
endpoint of every edge. Caterpillar graph is a denoted as $P(n,r_1, r_2,\dots r_n)$, where $r_i$ is the number of pendent vertices attached to $i^{th}$ vertex of $P_n$.
\end{definition}


\begin{lemma}
If G is a caterpillar graph graph then $\chi_{S1H}(G) = 3$.
\end{lemma}

\begin{figure}[htb]
\centering
\includegraphics[scale=0.5]{caterpillar.pdf}
\caption{\SH colouring using three colour on central path in caterpillar graph graphs}
\label{Figure: grid}
\end{figure}

\begin{proof}
If $P(n=3, r_1, r_2, r_3)$, where $r_i \geq 3$ and $\forall r_j=2$, $1 \leq j,i \leq 3$, and $j \neq i$ to dominate all leaves attached to the vertices on the central path, subset-1-harmonious colouring uses different colours to vertices on the central path. Otherwise if we colour all leaves of the vertex  $r_i \geq 3$, then we need more than three colours to dominate $r_i$. In general caterpillar graph, we can reuse the three colours of $r_1, r_2, r_3$ for all the vertices on the central path. Therefore $\chi_{S1H}(G) = 3$.

\end{proof}



==> chap3.tex <==
% chap3.tex


\chapter{Subset 1-Harmonious colouring}\label{chap:shc}


\section{Introduction}


\noindent
In this chapter, we initiate the study of a new colouring problem called \shar colouring. This problem is closely related to the previously discussed problem of \qCN colouring. Unlike the conflict-free colouring version, here the problem is restricted to having only distinct coloured neighbours, in case there are more than one colours present in the closed neighbourhood of a vertex $v$. The \shar colouring problem derives its motivation from the frequency allocation problem which avoids the presence of overlapping frequencies. Again, we consider the case of colouring a subset of vertices for \shar colouring.


\noindent
\textit{Formal Definition}: For a graph $G$, we define \shar colouring as a colouring function $c: V(G) \rightarrow \{c_0, c_1,\dots,c_q\}$ such that the following conditions are satisfied:
\begin{itemize}

	\item For every vertex $v$ and every colour $c_i$, $1 \leq i \leq q$, we have $|c^{-1}(c_i)\cap N[v]| \leq 1$.
	
	\item A vertex $v$ can have at most $deg[v] - 1$ number of vertices with colour $c_0$ in $N[v]$.
	
\end{itemize}


\noindent
We use $q$ colours $c_1, c_2,\dots,c_q$ to colour the graph $G$. However, as we are allowed to have some vertices uncoloured, we denote them to possess colour $c_0$. It is implicit that colour $c_0$ can repeat in closed neighbourhood of a vertex. A graph is said to be \shar coloured using $k$ colours if such a colouring exists. For a given graph $G$, let $\chi_{S1H}(G)$ represent the minimun value of $q$ such that there exists a \shar colouring of $G$ using $q$ colours.

\noindent
The objective that we accomplish in \shar colouring problem is the minimization of the number of colours used to colour a given graph. Let us now explore the problems that are similar to \shar colouring problem.



\noindent
\textit{Related Problems}: The problem of \textsc{Harmonious} colouring, was first introduced in 1983 by Hopcroft and Krishnamoorthy \cite{Harmonious} which was defined as follows: The harmonious chromatic number of a graph $G$, denoted by $h(G)$, is the least number of colours which can be assigned to the vertices of $G$ such that each vertex has exactly one colour, adjacent vertices have different colours, and any two edges have different colour pairs, as defined in \cite{Harmonious}. Later, \cite{dHarmonious} developed the concept of $d-$\textsc{Local Harmonious Chromatic} problem which generalized the \textsc{Harmonious Chromatic} problem. The $d-$\textsc{Local Harmonious} (or just $d$-\textsc{Harmonious}) chromatic problem imposes a restriction that the different colour-pair requirement is only asked to be satisfied for every edge within distance $d$ for any vertex. \shar colouring can be viewed as a variant of 1-\textsc{Harmonious} colouring where some vertices can be left uncoloured.

\noindent
Another colouring problem that is closely associated with \shar colouring is the problem of $L(d_1,d_2,\dots,d_k)$-\textsc{Labeling}, which is a non-negative integer vertex colouring such that the labels on vertices at distance $i$ differ by at least $d_i$. Therefore, $L(1,1)$-\textsc{Labeling} involves colouring of vertices with nonnegative integers such that the labels on adjacent vertices differ by at least 1 and the labels on vertices at distance 2 also differ by at least 1. This problem was initially introduced by Jerrold R. Griggs and Roger K. Yeh in the specific version of $L(2,1)$-\textsc{Labeling} \cite{yeh} and was later generalized to accommodate upto distance $k$, that is, $L(d_1,d_2,\dots,d_k)$. Our problem of \shar labeling is closely related to $L(1,1)$-\textsc{Labeling}. More specifically, in our problem we colour a subset of vertices of a given graph.

\noindent
The problem of \textsc{Efficent Dominating Set} for a given graph is also of interest while we study \shar colouring problem. An \textsc{Efficent Dominating Set} is one which is simultaneously an \textsc{Independent} and a \textsc{Perfect Dominating Set}. A \textsc{Perfect Dominating Set} $P$ is one in which each vertex $v \in V(G)$ has exactly one neighbour in $N(v)$ that belongs to $P$. Whereas an \textsc{Independent Dominating Set} $I$ satisfies the condition that set of vertices in $I$ form an independent set. Specifically, \textsc{Efficent Dominating Set} is a special case of \shar colouring. In other words, \textsc{Efficient Dominating Set} is same as \shar colouring when the number of colours used is 1.


\noindent
\textbf{Our Results}
\begin{enumerate}
	\item We give an upper bound on the number of colours required to \shar colour the following graph classes: complete graph, path, cycle, threshold graph and tree. Further, we bound the number of colours used to \shar colour the graph with respect to graph parameters such as maximum degree, vertex cover size, size of cluster vertex deletion set, neighbourhood diversity number and modular width.
	
	\item We present FPT algorithms for \shar colouring parameterized by structural parameters which include treewidth \& number of colours, size of vertex cover and neighbourhood diversity number.

\end{enumerate}


\noindent
We now begin the chapter by studying the bounds of \shar colouring for some classes of graphs. We then present fixed parameter tractable algorithms for \shar colouring when parameterized by certain parameters.




\section{Bounds on the number of colours for \shar colouring}

\noindent
Let us familiarize ourselves with \shar colouring with the help of some classes of graphs. We present the upper bound on the number of colours required to \shar colour these graph classes. The graphs that we study include complete graph, path, cycle, threshold graph and trees. These are followed by bounds on the number of colours used to colour graph $G$ when we consider certain graph parameters such as maximum degree of $G$, size of vertex cover of $G$, cluster vertex deletion number and modular width of $G$.


\subsection{Bounds for \shar colouring with respect to some classes of graphs}



\begin{definition}
Consider a graph $G$ on $n$ vertices. A complete graph $K_n$ is a graph $G$ on $n$ vertices with an edge between any two vertices $u,v \in V(G)$.
\end{definition}

\noindent
Let us analyse the number of colours required to \shar colour a complete graph $K_n$.


\begin{lemma}\label{completeG}
If G is a complete graph on n vertices then $\chi_{S1H}(G) = 1$.
\end{lemma}

\begin{proof}
The graph $K_n$ has each vertex adjacent to every other $n - 1$ vertices in the graph. Therefore, by assigning a colour to any one vertex of the graph will ensure that each vertex $v \in K_n$ is adjacent to the vertex that is assigned a colour. So this gives us a \shar colouring of $K_n$ such that $\chi_{S1H}(G) = 1$.
\end{proof}


\begin{lemma}
If $G$ is a path on n vertices then $\chi_{S1H}(G) = 1$.
\end{lemma}
\begin{proof}
Any path on $n$ vertices requires exactly one colour to be \shar coloured. We give a constructive proof of this. Consider a path $P_n$ such that it has $3k$ or $3k + 2$ vertices where $k \geq 1$. We can colour every third vertex beginning from the second vertex from one of the end vertices of the path. For path of length $3k+1$, we can colour the first vertex using colour 1 and every third vertex using the same colour and so on. This ensures that every vertex is dominated by exactly one coloured neighbour in its closed neighbourhood.
\end{proof}



\begin{lemma}
If G is a cycle on 3n vertices then $\chi_{S1H}(G) = 1$. Further, if G is a cycle on $3n + 1$ or $3n + 2$ vertices then $\chi_{S1H}(G) = 2$.
\end{lemma}
\begin{proof}
For a cycle on $3n$ vertices, we colour every third vertex and hence get a \shar colouring using 1 colour. For cycles on $3n+1$ and $3n+2$ vertices, we use colour 1 to colour every third vertex beginning from a vertex, say $v_1$, and finally use colour 2 to colour the last vertex that appears in this sequence. 


Furthermore, we note that one colour is not sufficient for cycles on $3n + 1$ or $3n + 2$ vertices. Consider a cycle on $3n+1$ vertices. To \shar colour this cycle using one colour, we start by colouring vertex $v_1$ and assign the same colour to every third vertex. We observe that the vertex $v_n$ is also assigned the same colour as $v_1$, which does not \shar colour vertices $v_1$ and $v_n$. Therefore, to avoid this conflict, we colour vertex $v_n$ using a new colour. Now consider a cycle on $3n+2$ vertices. We colour the vertices using one colour, as it was done for cycles on $3n+1$ vertices. We observe that vertices $v_1$ and $v_{n-1}$ of the cycle on $3n+2$ vertices are coloured using the same colour. So, to dominate vertex $v_n$, we assign it a new colour. Therefore, for cycles on $3n+1$ and $3n+2$ vertices, we have $\chi_{S1H}(G) = 2$.
\end{proof}



\noindent
Now we study the nature of \shar colouring with resepect to threshold graphs.

\begin{definition}
\cite{golumbic} A graph is a threshold graph if it can constructed from the empty graph by repeatedly adding either an isolated vertex or a dominating vertex.
\end{definition}


\begin{lemma}
If G is a threshold graph then $\chi_{S1H}(G) = 1$.
\end{lemma}

\begin{proof}
If isolated vertices are present, colour them using the same colour. By colouring the last introduced dominating vertex $v$, we satisfy \shar colour $G$ as each vertex in $G$ has only one coloured vertex $v$ in its closed neighbourhood.
\end{proof}


\begin{lemma}\label{treebound}
Let $\Delta$ be the maximum degree of a tree. Then $\Delta$ colours are sufficient to \shar colour the tree. Moreover, $\Delta-1$ colours are sometimes necessary.
\end{lemma}
\begin{proof}
Consider a tree $T$ with a root $r$. Colour root $r$ with a colour $c_i$ where $i \neq 0$. The nodes present in its next level are left uncoloured. The nodes in following level (i.e., grandchildren of $r$) are coloured using colours $c_j$ where $j \not\in \{0,i\}$ and each of the nodes adjacent to each child of $r$ recieve a different colour. Such an assignment is accomplished due to the fact that we have $\Delta - 1$ colours after colouring $r$ with $c_i$. This preserves the characteristic of \shar colouring by assigning at most $\Delta$ unique colours to the vertices in the closed neighbourhood of each node of $T$. In other words, we colour alternate levels of a tree to \shar colour it. Therefore, either a vertex $v$ is coloured or all its neighbours are coloured using at most $\Delta$ colours.

\noindent
We remark that this may not be the optimal colouring in terms of number of colours used. However, this serves as an upper bound on the number of colours required to \shar colour a tree.

\noindent
To prove the lower bound, consider a tree $T$ of height 2. Let $r$ be the root and $d$ be the number of children of each vertex in $T$, except leaves. Therefore, maximum degree $\Delta = d + 1$. Let $v$ be a vertex at height 1. Note that to \shar colour the children of $v$, we need $d$ colours if we colour each child of $v$ using a different colour. Otherwise we have to colour $v$ in order to dominate uncoloured child node(s) of $v$. By extending this argument for each of $d - 1$ siblings of $v$, any \shar colouring of $T$ use $d$ colours. Thus the lower bound follows. Refer Figure \ref{Figure: label_sharTree}.


\end{proof}


\begin{figure}[htb]
\centering
\includegraphics[scale=0.7]{Images/sharTree.pdf}
\caption{\shar colouring tree $T$ with $d=3$}
\label{Figure: label_sharTree}
\end{figure}


\noindent
We observe that to \shar colour tree $T$ in above construction requires $\Omega(\sqrt{n})$ vertices to be coloured. Hence, we state the following corollary.


\begin{coro}
There exist trees that require $\Omega(\sqrt{n})$ number of vertices to be coloured so that the tree is \shar coloured.
\end{coro}





\noindent
Until now, we have explored the bounds for \shar colouring graph $G$ with respect to special graph classes, namely complete graph, path, cycle, threshold graph and trees. We will now examine \shar colouring with respect to some graph parameters. We consider the following graph parameters: maximum degree, treewidth, vertex cover size, cluster vertex deletion number, neighbourhood diversity number and modular width. Note that the upper bounds for \shar colouring with respect to the said graph parameters are studied for a general graph $G$.




\subsection{Bounds for \shar colouring with respect to graph parameters}




\noindent
The first graph parameter that we study is the maximum degree $\Delta$ of graph $G$. Let us analyse the behavior of graph $G$ for \shar colouring with respect to $\Delta$.


\begin{lemma}
Let $\Delta$ be the maximum degree of a graph $G$. There exists a \shar colouring of $G$ such that $\chi_{S1H}(G)\leq\Delta^2+1$.
\end{lemma}
\begin{proof}
\noindent
For a given graph $G$, we construct graph $G^2$ as follows. The vertices $V(G^2)$ are same as vertices $V(G)$. We retain the edges of $E(G)$ in $E(G^2)$. Further, consider two non adjacent vertices $u$ and $v$ in $G$. If there exists a vertex $w$ that is adjacent to both $u$ and $v$, then add an edge $uv$ to graph $G^2$. This is done for every pair of distance-2 vertices $u$ and $v$ to get edge set of graph $G^2$. We observe that proper colouring of graph $G^2$ gives us a \shar colouring for graph $G$. Therefore, number of colours required to \shar colour graph $G$ is $\chi(G^2) \leq \Delta^\prime + 1$, where $\Delta^\prime$ is the maximum degree of a vertex in $G^2$. Since $\Delta^\prime$ is at most $\Delta^2$, the result follows.

\end{proof}



\noindent
The next parameter of interest is the treewidth of graph $G$. Treewidth is a measure of how close a graph is to a tree-like structure. However, with respect to this parameter, it is uncertain to predict the behavior of \shar colouring when we try to capture the number of colours required for $G$. Consider the case of complete graphs. As described in Lemma \ref{completeG}, the number of colours required to \shar colour a complete graph is 1. However, its treewidth is $O(n)$. On the other hand, we note that there exist trees, although the treewidth being 1, such that $\chi_{S1H}\geq\sqrt{n}$, as proved in Lemma \ref{treebound}. Let us now examine vertex cover as a parameter of $G$ which is larger then treewidth.


\begin{lemma}\label{sharVCbound}
The number of colours required to \shar colour the vertices of graph G  is at most the size of vertex cover of $G$, that is, $\chi_{S1H}(G)\leq \textsc{VC(G)}$.
\end{lemma}

\begin{proof}
We know that every edge $e \in E(G)$ has at least one of its end vertices in vertex cover of $G$. Consider a graph $G$ with a vertex cover $X$ of size $k$. Firstly, assign one of the $k$ colours to all isolated vertices, if they exist. Next assign different colours to each vertex that form the vertex cover of $G$. Therefore, we have utilized $k$ colours to colour vertices in $X$ as the size of $X$ is $k$. This \shar colours the vertices in $X$. By the definition of vertex cover of $G$, each edge $e \in E(G)$ has at least one of its end vertices in vertex cover and hence it is coloured by one of the $k$ colours. Since we colour each vertex of $X$, we are sure that vertices in $V(G)\backslash X$ will be adjacent to at least one of the coloured vertices in $X$. Moreover, each vertex in $X$ is coloured using a different colour which avoids overlapping of colours. Therefore, we can conclude that every vertex $v \in V(G)$ has a coloured vertex in its closed neighbourhood. Further, in the presence of more than one coloured neighbour, we can be assured of the colour being distinct as all the vertices in $X$ as coloured using $k$ different colours, hence satisfying \shar colouring of $G$.

\end{proof}





\noindent
We proceed to understand the nature of \shar colouring with respect to  the the size of cluster vertex deletion set of graph $G$ which is a smaller parameter compared to vertex cover of $G$.


\begin{definition}
A cluster graph is a disjoint union of complete graphs.
\end{definition}

\begin{definition}
A cluster vertex deletion set $X$ of a graph $G$ is a set of vertices such that $G\backslash X$ forms a cluster graph.
\end{definition}
\noindent
The cluster vertex deletion number is defined as the minimum possible size of cluster vertex deletion set $X$. Intuitively, it is the measure of how close a graph is to being a cluster graph.


\begin{lemma}\label{sharCVDSbound}
Let $X$ be a cluster vertex deletion set of graph $G$. Then $\chi_{S1H}(G)\leq |X|+1$.
\end{lemma}
\begin{proof}
To \shar colour graph $G$, we colour each vertex $v \in X$. If the size of $X$ is $k$, then we have utilized $k$ colours. Now colour exactly one of the undominated vertices in each complete graph(s) in $G\backslash X$ using a colour that is different from previously used $k$ colours. Note that two coloured vertices $u$ and $v$ in two different cluster graphs do not have a common neighbour in $X$ because in such a scenario, we would not choose either of $u$ or $v$ to assign it the $(k+1)^{th}$ colour. We assign $(k+1)^{th}$ colour to an $undominated$ vertex in each cluster graph which implies that this vertex is not adjacent to any vertex in $X$. This gives us a \shar colouring of $G$ as the vertices in $X$ are dominated by the colours assigned to them. Additionally, some of the vertices in $G\backslash X$ may also have a neighbour in $X$. Every $v \in V(G)$ has at least one coloured neighbour in $N[v]$ and in case more than one coloured vertices are present in $N[v]$, we are assured of them being distinct because we have used $k+1$ colours. Therefore the result follows.
\end{proof}



\noindent
The next graph parameter for study of \shar colouring is the neighbourhood diversity of $G$.

\begin{definition}
\cite{gargano2015complexity} Given a graph $G = (V,E)$, two vertices $u,v \in V$ have the same type if and only if $N(v)\backslash\{u\} = N(u)\backslash\{v\}$. The graph $G$ has a \textit{neighbourhood diversity t}, if there exists a partition of $V$ into at most $t$ sets, $V_1, V_2,\dots,V_t$ such that all the vertices in $V_i$ have the same type for $i = 1,2,\dots,t$. The family $\nu = \{V_1,V_2,\dots,V_t\}$ is called the type partition of $G$.
\end{definition}
\noindent
On creating such a type partition of $V(G)$, we observe that the vertices within a partition either form a complete graph or an independent set. Further, for $1 \leq i, j \leq t$, each vertex in a partition $V_i$ is either adjacent to every vertex in another partition $V_j$ or there are no edges between vertices of $V_i$ and $V_j$.


\begin{lemma}\label{sharNDbound}
The number of colours required to \shar colour a graph $G$ is at most its neighbourhood diversity, that is, $\chi_{S1H}(G)\leq t$.
\end{lemma}
\begin{proof}
For a given graph $G$, consider its type partition $\nu$ with neighbourhood diversity $t$. Colour all isolated vertices, if any, using one of the $t$ colours. For $1 \leq i \leq t$, colour a vertex in each $V_i$ using a different colour. By doing so we \shar colour $V(G)$. This can be justified as follows. Partitions $V_i$ that form a complete graph are all dominated due to the presence of a coloured neighbour in $V_i$. Additionally, if vertices of $V_i$ are adjacent to partition $V_j$ for $1 \leq j \le t$, we can expect them to be adjacent to some more coloured neighbours. Now consider the case where vertices in partition $V_i$ form an independent set. If vertices in partition $V_i$ are not isolated vertices, then they will be adjacent to all vertices of another partition $V_j$ which assures the presence of at least one coloured neighbour in the closed neighbourhood of each vertex in $V_i$. Hence we have used $t$ number of colours to \shar colour $G$.
\end{proof}



\noindent
We conclude this section on bounds on the number of colours for \shar colouring by studying the problem for modular width of $G$. The modular width of graph $G$ is computed by virtue of four operations, namely creation of isolated vertex, disjoint union, complete join and substitution. More precisely, the modular width of $G$ equals the maximum number of operands used by any occurrence of  substitution operation. These four operations that are involved in modular decomposition of graph $G$ are described in \cite{modularwidth}. For the sake of completeness, we mention the four operations here.

\begin{definition}\label{mod_def} \cite{modularwidth} Algebraic operations involved to compute modular width of graph $G$.
\begin{itemize}
\item Create an isolated vertex;
\item The disjoint union of two graphs, i.e., the \textit{disjoint union} of two graph $G_1$ and $G_2$, denoted by $G_1 \otimes G_2$, is the graph with vertex set $V(G_1)\cup V(G_2)$ and edge set $E(G_1)\cup E(G_2)$;
\item The complete join of two graphs, i.e., the \textit{complete join} of two graphs $G_1$ and $G_2$, denoted by $G_1\oplus G_2$, is the graph with vertex set $V(G_1)\cup V(G_2)$ and edge set $E(G_1)\cup E(G_2)\cup \{ \{v, w\}: v\in V(G_1)$ and $w\in V(G_2)\}$.
\item The substitution operation with respect to some graph $G$ with vertices $v_1,\dots,v_n$, i.e., for graphs $G_1,\dots,G_n$ the substitution of the vertices of $G$ by the graphs $G_1,\dots,G_n$, denoted by $G(G_1,\dots,G_n)$, is the graph with vertex set $\underset{1 \leq i \leq n}\cup V(G_i)$ and edge set $\underset{1 \leq i \leq n} \cup E(G_i)\cup \{\{u, v\}:u \in V(G_i)$ and $v \in V(G_j)$, $v_i,v_j \in E(G)$ and $i\neq j\}$. Hence, $G(G_1,\dots,G_n)$ is obtained from $G$ by substituting every vertex $v_i \in V(G)$ with the graph $G_i$ and adding all edges between the vertices of a graph $G_i$ and the vertices of a graph $G_j$ whenever $\{v_i, v_j\} \in E(G)$.
\end{itemize}
\end{definition}

\begin{definition} \cite{modularwidth} Let A be an algebraic expression that uses only the four operation as mentioned in Definition \ref{mod_def}. We define the width of A as the maximum number of operands used by any occurrance of the substitution operation in A. Modular width of graph G, denoted as mw(G), is the least integer m such that G can be obtained from such an algebraic expression of width at most m.

\end{definition}


\begin{lemma}
The maximum number of colours required to \shar colour $G$ equals the modular width of the graph, that is, $\chi_{S1H}(G)\leq mw(G)$.
\end{lemma}
\begin{proof}
Let us now examine the maximum number of colours required to \shar colour $G$ while we perform each of the above mentioned operations, in that sequence. On introducing an isolated vertex, we \shar colour it by using one colour. To dominate the vertices created as a result of disjoint union of vertices, we would require the maximum of all colours that was used in each component of disjoint sets. The complete join operation involves introducing edges between the two sets of vertices on which we intend to perform a complete join. Edges are introduced between every pair of vertices of the two sets of vertices, in addition to the existing edges. By using exactly two colours and colouring one vertex in each partition, we \shar colour all vertices introduced thus far. Finally, we examine the fourth operation, that is substitution. In the substitution operation, we replace each vertex $v_i \in V(G)$ with the graph $G_i$ and adding all edges between the vertices of a graph $G_i$ and the vertices of a graph $G_j$ whenever $\{v_i,v_j\}\in E(G)$ \cite{modularwidth}. We colour one vertex in each $G_i$. Besides the presence of coloured neighbour(s) in $G_i$, a vertex may possibly be adjacent to another coloured vertex in $G_j$. To \shar colour $G$, we would then require the number of operands in this operation.
\end{proof}








\section{FPT Algorithms for \shar colouring}



\noindent
In this section, we study the following decision version of the \shar colouring problem. Given a graph $G$ can we \shar colour $G$ using at most $q$ colours?

\noindent
As mentioned earlier in this chapter, the problem of \textsc{Efficient Dominating Set} is a special case of \shar colouring when $q=1$. However, the problem of finding an \textsc{Efficient Dominating Set} is NP-complete \cite{effdom}. Hence, the problem of \shar colouring is also NP-complete. Therefore, we explore the possibility of algorithms that are fixed parameter tractable to find \shar colouring of a graph. But with respect to the standard parameter $q$, the problem is para-NP-hard since it is NP-complete even for $q=1$. So we investigate the problem of \shar colouring parameterized by structural parameters. One of the common and well studied structural parameter is treewidth of the graph. The next lemma states the result for parameterization by treewidth.



\begin{lemma}\label{twW1}
\shar colouring parameterized by treewidth of a graph is W[1]-hard.
\end{lemma}

\begin{proof}
Another problem that we said is closely related to \shar colouring is the problem of \textsc{L(1,1)-Labeling}. Theorem 5 of \cite{petr} proves that \textsc{L(1,1)-Labeling} problem is W[1]-hard parameterized by treewidth. They give a parameterized reduction from the \textsc{Equitable colouring} problem to the \textsc{L(1,1)-Labeling} problem. We modify the reduction as follows to get an instance of the \shar colouring problem. To the reduced graph $H$ in Theorem 5 of \cite{petr}, we add $q+1$ number of degree-1 vertices to each $v \in V(H)$ to obtain graph $H^\prime$. This forces all the vertices in $V(H)$ to be coloured since otherwise we would colour each of the $q+1$ vertices that we introduced in graph $H^\prime$, which clearly overshoots the given budget of $q$ colours. Further, note that this modification does not alter the treewidth of $H$. Therefore, \shar colouring problem parameterized by treewidth is $W[1]$-hard.
\end{proof}


\noindent
We now explore the possiblity of parameterization by treewidth $\tau$ and the number of colours $q$.





\subsection{\shar colouring parameterized by treewidth and number of colours}

\noindent
We study \shar colouring when parameterized by treewidth and number of colours. Courcelle's Theorem \cite{courcelle1990monadic} states that every graph property definable in the monadic second-order logic of graphs can be decided in linear time on graphs of bounded treewidth. By Courcelle's theorem it can proved that \shar colouring parameterized by treewidth and number of colours has an FPT algorithm. Here we give a constructive proof for the same.

\begin{proposition}\label{tw-compute}
Given a graph $G$, in time $O(2^{O(\tau)}n)$, we can compute a nice tree decomposition $(T,{\cal X})$ of $G$ with $|V(T)| \in |V(G)^{O(1)}|$ and of width at most $5\tau$, where $\tau$ is the treewidth of $G$ \cite{5tw}.
\end{proposition}

\noindent
We design a fixed parameter tractable algorithm for \shar colouring problem. We give an algorithm based on dynamic programming over nice tree decomposition. The algorithm starts by computing a nice tree decomposition $(T,{\cal X})$ of $G$ in time $O(2^{O(\tau)}n)$, using Proposition~\ref{tw-compute}, of width at most $5\tau$, where $\tau$ is the treewidth of $G$. We define subproblems on $t \in V(T)$ for the graph $G_t$. We consider a \textit{partitioning} of bag $X_t$ by a mapping $f : X_t \rightarrow \{B, W, R\}$. For simplicity, we refer to the vertices in each partition respectively as black, white and grey. Each vertex is also assigned another colour by a function $c$ : $X_{t} \rightarrow \{ c_0,c_1,...,c_q \}$ and a $q$-length tuple, by a function $\Gamma$: $X_{t} \rightarrow \{ 0,1,\hat{1} \}^q$. Roughly speaking, these functions will determine how the ``partial'' conflict-free colouring looks like, when restricted to $G_t$ and vertices of $X_t$. $c(v)$ denotes the colour assigned to $v$ and $c(v)=c_0$ denotes that $v$ is not coloured. $\Gamma(v)[i]$ indicates whether $v$ has (either in the current graph, or in the ``future'') a vertex in its closed neighbourhood that has colour $c_i$. $\Gamma(v[i]) = 1$ denotes that vertex $v$ has a vertex in its closed neighbourhood of colour $c_i$ in $G_t$, $\Gamma(v)[i] = \hat{1}$ denotes that vertex $v$ has a vertex in its closed neighbourhood of colour $c_i$, that is not present in $G_{t}$, but will appear in the ``future'', and $\Gamma(v)[i] = 0$ denotes the absence of colour $c_i$ in the closed neighbourhood of $v$. We slightly abuse the notation sometime and use $\Gamma(v)[c_i]$ and $\Gamma(v)[i]$ interchangeably. In the following we give a detailed insight into the functions $f$, $c$ and $\Gamma$.
\\\noindent \textbf{Black}, represented by $B$. Every black vertex $v$ is given a colour $c(v) \neq c_0$ in a \shar colouring.
\\\noindent\textbf{Grey}, represented by $R$. A grey vertex $v$ is not coloured, not dominated, i.e. $c(v) = c_0$ and for each $i \in [q]$, it has $\Gamma(v)[i] \in \{0,\hat 1\}$. 
 \\\noindent\textbf{White}, represented by $W$. A vertex $v$ that is neither black nor grey is a white vertex. Note that for a white vertex $v$, $c(v) =c_0$ and there is $i \in [q]$, such that $\Gamma(v)[i]=1$. 

\noindent
As our goal is to only show whether or not the problem is FPT, we did not try to optimise the running times. 
A tuple $(t,c,\Gamma,f)$ is \emph{valid} if the following conditions hold for every vertex $v \in X_t$:
\begin{enumerate}
	\item $f(v)=B \implies c(v) \ne c_0$ and $\Gamma(v)[c(v)] = 1$, 		\item $f(v)=R \implies c(v)=c_0$ and $\Gamma(v)[i] \in \{0,\hat{1}\}$, $\forall i \in \{1...q\}$, and iii) $f(v)=W \implies c(v)=c_0$ and $\Gamma(v)[i] = 1$ for some $i \in \{1...q\}$.
\end{enumerate}

\noindent
For a node $t\in V(T)$, for each valid tuple $(t,c,\Gamma,f)$, we have a table entry denoted by $D[t,c,\Gamma, f]$. We have $D[t,c,\Gamma, f]= true$ if and only if there is ${\sf col} : V_t \rightarrow \{c_0,c_1,\ldots, c_q\}$ (where $c_0$ denotes no colour assignment), such that: 
\begin{enumerate}
	\item ${\sf col}|_{X_t} = c$,
	\item for each $v \in X_t$ and $i\in \{1,2,\dots q\}$ with $\Gamma(v)[i] = 1$, there is exactly one vertex $u\in N_{G_t}[v]$, such that $\col(u) = c_i$,
	\item for each $v \in X_t$ and $i\in [q]$ with $\Gamma(v)[i] \in \{0,\hat 1\}$, there is no vertex $u \in N_{G_t}[v]$, such that $\col(u) = c_i$, and
	\item for each $v\in V_t \setminus X_t$, there is a vertex $u\in N_{G_t}[v]$, such that $\col(u) \neq c_0$, and for every other $u' \in N_{G_t}[v]$ we have ${\sf col} (u^\prime) \neq {\sf col}(u)$.
\end{enumerate}


\noindent
In the above, such a colouring $\col$ is called a $(t,c,\Gamma,f)$-\emph{good} colouring. (At any point of time wherever we query an invalid tuple, then its value is $false$ by default.) 
 Note that $D[r,\phi,\phi,\phi] = true$, where $r$ is the root of the tree decomposition, if and only if $G$ admits a \shar colouring using (at most) $q$ colours. 
\noindent We now proceed to define the recursive formulas for the values of $D$. \\
\noindent\textbf{Leaf node.} For a leaf node $t$, we have $X_t = \emptyset$. Hence, the only entry is $D[t, \phi, \phi, \phi]$. Moreover, by definition, we have $D[t, \phi, \phi, \phi] = true$.\\
\noindent\textbf{Introduce vertex node.} Let $t$ be the introduce vertex node with a child $t'$ such that $X_t = X_{t'} \cup \{v\}$ for some $v \not\in X_{t'}$. Since the vertex $v$ is isolated in $G_t$, the following recurrence follows.
\begin{align*}
    D[t, c, \Gamma, f] = &
    \begin{cases}
    D[t', c_{|X'}, \Gamma_{|X'}, f_{|X'}] \text{ if } & f(v) = B \text{ and } \Gamma(v)[c_i] \in \{0,\hat{1}\} \text{ }, \forall \text{ } c_i \neq c(v)\\
    D[t', c_{|X'}, \Gamma_{|X'}, f_{|X'}] \text{ if } & f(v) = R \\
    \text{False } & \text{otherwise}
    \end{cases}
\end{align*}

\noindent\textbf{Introduce edge node.} Let $t$ be an introduce edge node labeled with an edge $u^*v^*$ and let $t'$ be the child of it. Thus $G_{t'}$ does not have the edge $u^*v^*$ but $G_t$ has. Consider distinct $u,v\in \{u^*,v^*\}$. 
\begin{enumerate}
\item If $f(u)=B$, $f(v)=W$ and $\Gamma(v)[c(u)] = 1$. We set $D[t, c, \Gamma, f]= D[t', c,$ $ \Gamma_{v[c(u)]\rightarrow \hat{1}}$, $f_{v\rightarrow R}] \vee D[t', c, \Gamma_{v[c(u)]\rightarrow \hat{1}}$, $f_{v\rightarrow W}]$ (if any of the entries are invalid, then it is $false$). 
\item If $f(u)=f(v)=B$ and $ \Gamma(v[c(u)]) = \Gamma(u[c(v)]) = 1$, set $D[t, c, \Gamma, f]= D[t', c, \Gamma_{v[c(u)]\rightarrow\hat{1},u[c(v)]\rightarrow\hat{1}}, f] $.
\item If $\{f(u),f(v)\} \cap \{B\} = \emptyset$, then $D[t, c, \Gamma, f]=D[t', c, \Gamma, f]$.
\item If none of the above conditions hold then $D[t, c, \Gamma, f]=false$.
\end{enumerate}
\begin{lemma}
Recurrence for introduce edge node is correct.
\end{lemma}
\begin{proof}
Note that all the vertices except $u$ and $v$ in $X_t$ are unaffected by introduction of edge $u^*v^*$. Also if neither $u$ nor $v$ are black, then the edge $uv$ cannot \shar dominate any vertex. Therefore the value of $D$ for that tuple is same as that in the child node. Consider the case where $f(u) =B$ and $f(v)=W$ and  $\Gamma(v)[c(u)] = 1$. We show that $D[t,c,\Gamma,f]=true$ when at least one of $D[t^\prime,c,\Gamma_{v[c(u)]\rightarrow \hat{1}},f_{v\rightarrow R}]$ and $D[t^\prime,c,\Gamma_{v[c(u)]\rightarrow \hat{1}},f]$ is $true$. Let $D[t^\prime,c,\Gamma_{v[c(u)]\rightarrow \hat{1}},f_{v\rightarrow R}]=true$. Let $\col : V_{t\prime} \rightarrow \{c_0,\dots,c_q\}$ be a $(t^\prime,c,\Gamma_{v[c(u)]\rightarrow \hat{1}},f_{v\rightarrow R})$-good colouring in $G_{t^\prime}$. Note that $\col(v) =c_0$ and there is no vertex $v' \in N_{G_{t'}}[v]$ such that $\col(v')=c(u)$. Therefore, $\col$ is also a $(t,c,\Gamma,f)$-good colouring since $u$ is the unique vertex in $N_{G_t}[v]$ with $\col(u)=c(u)$. 
 Hence $D[t,c,\Gamma,f]=true$. Similarly, we can prove that when $D[t^\prime,c,\Gamma_{v[c(u)]\rightarrow \hat{1}},f]=true$, any $(t^\prime,c,\Gamma_{v[c(u)]\rightarrow \hat{1}},f)$-good colouring is also a $(t,c,\Gamma,f)$- colouring. In the reverse direction, assume  $D[t,c,\Gamma,f]=true$ and let $\col : V_{t} \rightarrow \{c_0,\dots,c_q\}$ be a $(t,c,\Gamma,f)$ - good colouring. Therefore, $u$ is the unique vertex in $N_{G_t}[v]$ such that $\col(u)=c(u)$. If there exists a $c_i \ne c(u)$ such that $v$ has a neighbour $v'$ in $N_{G_t}[v]$ with $\col(v')=c_i$, then $\col$ is a $(t^\prime,c,\Gamma_{v[c(u)]\rightarrow \hat{1}},f)$-colouring, otherwise  $\col$ is a $(t^\prime,c,\Gamma_{v[c(u)]\rightarrow \hat{1}},f_{v\rightarrow R})$-colouring. We can prove the correctness for other cases by similar arguments.

\end{proof}
\textbf{Forget node.} Let $t$ be a forget node with child $t'$ such that $X_t = X_{t'} \setminus \{v\}$ for some $v \in X_{t'}$. Since the vertex $v$ does not appear again in any bag of a node above $t$, $v$ must be either black or white (otherwise, we set the entry to $false$). %This gives the following recursive formulas for all vertices $v \in V(G) $: 
\begin{align*}
    D[t, c, \Gamma, f] =  \bigvee_{\substack{1 \leq i \leq q \\ \alpha \in \{0,1\}^q}} \left( D[t', c_{v\rightarrow c_0}, \Gamma_{v\rightarrow\alpha}, f_{v\rightarrow W}]   \vee  D[t', c_{v\rightarrow c_i}, \Gamma_{v\rightarrow\alpha}, f_{v\rightarrow B}] \right)
\end{align*}
\iffalse
\begin{align*}
    d[t, c^1, c^2, f] = & \left( \lor_{i=1}^q d[t', c^1_{w\rightarrow 0}, c^2_{w \rightarrow i}, f_{w\rightarrow 0}] \right)  \lor  \left( \lor_{i=1}^q d[t', c^1_{w\rightarrow j}, c^2_{w \rightarrow i}, f_{w\rightarrow 1}] \right)
\end{align*}
\fi
\\
\textbf{Join node.} Let us denote the the join node by $t$. Let $t_1$ and $t_2$ be the children of $t$. We know that $X_t = X_{t_1} = X_{t_2}$ and $X_t$ induces an independent set in the graphs $G_t$, $G_{t_1}$ and $G_{t_2}$. We say that the pair of tuples $[t_1,f_1,c_1,\Gamma_1]$ and  $[t_2,f_2,c_2,\Gamma_2]$ are $[t,f,c,\Gamma]$-consistent if for every $v \in X_t$ the following conditions hold.
\begin{itemize}
\item  If $f(v) = B$ then $(f_1(v), f_2(v)) = (B,B)$ and $c_1(v) = c_2(v)=c(v)$. 
\item  If $f(v)=W$ then $(f_1(v), f_2(v)) \in \{(W,R),(R,W),(W,W)\}$.
\item  If $f(v) = R$ then $(f_1(v),f_2(v))=(R,R)$. 
\item  If $\Gamma(v)[i] = 0$ then $(\Gamma_1(v)[i], \Gamma_2(v)[i]) \in \{(0,0)\}$ for $1 \leq i \leq q$.
\item  If $\Gamma(v)[i] = 1$ then $(\Gamma_1(v)[i], \Gamma_2(v)[i]) \in \{(1,\hat{1}),(\hat{1},1)$\} for $1 \leq i \leq q$.
\item   If $\Gamma(v)[i] = \hat{1}$ then $(\Gamma_1(v)[i], \Gamma_2(v)[i]) \in \{(\hat{1},\hat{1})\}$ for $1 \leq i \leq q$. 
\end{itemize}


\noindent
It is easy to see that a vertex $v$ belongs to Black partition in $X_t$ if it is Black in $X_{t_1}$ and $X_{t_2}$ and the colour $c(v)$ that is assigned to $v$ is same in these bags. Similarly, we can understand for a vertex in Grey partition. If vertex $v$ belongs to White partition, it implies that it is dominated in exactly one of bags $X_{t_1}$ and $X_{t_2}$ or both. However if $v$ is dominated in both the bags, then the colour that dominates it is different which is taken care by $\Gamma(v)[i]$. The value of $\Gamma(v)[i]$ is set to 1 for different values of the $q$-length tuple. Therefore, for a vertex to belong to White partition requires one of the three combinations: $\{(W,R),(R,W),(W,W)\}$. Now consider the values that $\Gamma(v)[i]$ can take in $X_t$. If colour $i$ is not present in $N[v]$ in any of the children nodes $t_1$ and $t_2$, then it will naturally not be present in $N[v]$ in $X_t$, implying $\Gamma(v)[i] = 0$. However, $\Gamma(v)[i] = 1$ indicates the presence of a vertex with colour $i$ in $N[v]$ in $X_t$. We further note that colour $i$ appears exactly in of the children $X_{t_1}$ or $X_{t_2}$ but not both because presence of colour $i$ in both children nodes will have two vertices with colour $i$ in $N[v]$ in $X_t$, which contradicts the conditions that satisfy \shar colouring. The next possibility of $\Gamma(v)[i]$ is $\hat{1}$. For this to be true, the colour $i$ should not be present in $G_t$ seen so far but will appear in the tree decomposition eventually.


\noindent
We set $ D[t, c, \Gamma, f] = \bigvee_{\substack{(f_1,f_2)}}\left({ D[t_1, c_1, \Gamma_1, f_1] \wedge D[t_2, c_2, \Gamma_2, f_2]} \right)$, \\ where $[t_1,f_1$, $c_1,\Gamma_1]$ and $[t_2,f_2,c_2,\Gamma_2]$ is $[t,f,c,\Gamma]$-consistent.

\noindent
We have described the recursive formulas for the values of $D[\cdot]$. Note that we can compute each entry in time bounded by $2^{O(q\tau)}\cdot  q^{O(\tau)} n^{O(1)}$. Moreover, the number of (valid) entries for a node $t\in V(T)$ is bounded by $2^{O(q\tau)}\cdot q^{O(\tau)} n^{O(1)}$, and $V(T) \in n^{O(1)}$. Thus we can obtain that the overall running time of the algorithm is bounded by $2^{O(q\tau)} n^{O(1)}$. Thus, we obtain the following theorem.

\begin{theorem}\label{thm:StrongCFC}
\shar is FPT when parameterized by the treewidth $\tau$ of the input graph and the number of colours $q$.
\end{theorem}




\subsection{\shar colouring parameterized by the size of vertex cover}\label{sharVC}

\noindent
We concluded in Lemma \ref{twW1} that \shar colouring is $W[1]$-hard when parameterized by treewidth. In this section we study an FPT algorithm for \shar colouring of graph $G$ when parameterized by the size of vertex cover of $G$. Vertex cover, a larger graph parameter than treewidth, accommodates tractable algorithms for \shar colouring. We study an FPT algorithm for \shar colouring for $G$ that uses $q$ colours. Let $X$ be a $k$-sized vertex cover of $G$. Note that if $q \geq k$, then by Lemma \ref{sharVCbound} it is trivially true that a \shar colouring exists. Therefore, we assume that $q < k$.


\begin{itemize}
\item Consider all possible $(q + 1)^k$ colourings of vertex cover\footnote{There are q colours and another possible colouring of a vertex \emph{v} in vertex cover is that it gets no colour. And there are \emph{k} vertices in vertex cover. Hence $(q + 1)^k$ colourings of vertex cover is possible.}. A subset of vertices in vertex cover may not be dominated due to absence of a coloured vertex in its closed neighbourhood. Therefore we require to colour the neighbour(s) of such vertices in $V(G)\backslash X$, which forms an independent set. Let us denote $V(G)\backslash X$ as $I$. Furthermore, there may be vertices in $I$ that may not be dominated and hence need to be coloured.


\item Consider a vertex $v \in X$ that is assigned colour $c_0$. The neighbours of vertex $v$ in $I$ need to be assigned a colour $c_i$, $1 \leq i \leq q$ unless they are already dominated by some other vertex in $X$. Observe that $v$ can have at most $q$ such neighbours in $I$, otherwise the colouring on $X$ does not support \shar colouring of graph $G$. We find vertices in $I$ with similar characteristic as that of neighbours of vertex $v$ in $I$ as call them as set of vertices $W$. The number of vertices in $W$ is therefore bounded by $q^2$ which is at most $k^2$ as $q \leq k$. We can now colour the vertices in $W$ in $\mathcal{O}(k^{k^2})$.


\item We will now be left with vertices in $X$ that are not dominated. We find the neighbours of such vertices in $I$ and call them as the set of vertices $U$. Note that if two or more vertices in $U$ have the same neighbourhood in $X$, then we retain exactly one such vertex in $U$. Including only one vertex $U$, among all vertices with same neighbourhood, is safe since the vertices that are not included can be coloured using the same colour as given to the vertex that is included in $U$. Since there are $2^k$ possible neighbourhoods of undominated vertices of $X$ in $I$, we colour the vertices of $U$ in $\mathcal{O}(q^{2^k})$ or $\mathcal{O}(k^{2^k})$ as $q \leq k$.


\end{itemize}



\noindent
Let us compute the running time of above algorithm. To colour a subset of vertices in vertex cover, we require $\mathcal{O}(k^k)$ time. The vertices in independent set that are assigned colour are categorized in to vertices $W$ and $U$ which are coloured in $\mathcal{O}(k^{k^2})$ and $\mathcal{O}(k^{2^k})$ respectively. Hence the running time is of the order of $\mathcal{O}(k^{2^k})$.





\subsection{\shar colouring parameterized by neighbourhood diversity number}

\noindent
We parameterize \shar colouring by neighbourhood diversity number of the graph $G$. We colour all the isolated vertices of $G$ using the same colour, if they exist. Now consider the type partitions of $G$, that is $V_1, V_2, \dots, V_t$. For the given neighbourhood diversity partition $t$, we construct a graph $H$ such that $|V(H)| = t$ and between any two vertices of graph $H$, there exists an edge if there are edges across corresponding partitions in graph $G$.

\noindent
From Lemma \ref{sharNDbound}, the number of colours $q$ that are required to \shar colour $H$ will be at most $t$. On colouring each vertex of $H$, we will correspondingly colour exactly one vertex in each partition $V_i$ in $G$ for $1 \leq i \leq t$. The colouring of $V(H)$ is accomplished by brute force in time $O(q^t)$. Since $q \leq t$, we obtain a running time of $O(t^t)$.



\section{Conclusion}

\noindent
In this chapter, we explored a new variant of graph colouring problem called \shar colouring. We explored the behaviour of this type of colouring for special graph classes such as complete graphs, path, cycle and trees; giving an upper bound on the number of colours required to colour these graph classes while satisfying \shar colouring. We further investigated the graph parameters such as maximum degree of graph, treewidth, vertex cover, cluster vertex deletion set, neighbourhood diversity and modular width. We concluded the chapter with fixed parameter tractable algorithms for \shar colouring with respect to structural parameters such as treewidth \& number of colours, size of vertex cover and neighbourhood diversity number.

==> conclusion.tex <==
\noindent
In this paper, we explored a new variant of graph colouring problem called \sh . We explored the behaviour of this type of colouring for special graph classes and giving an upper bound on the number of colours required to colour these graph classes while satisfying \sh. We proved that \sh using $2$ colors on planar bipartite is NP$-$complete. As an extension of this result if number of colors are $2$, then it can not preserve planarity.Since we prove that 
\sh using $q$ colors, where $q>2$ on bipartite is NP$-$complete.
We concluded the paper with parameterized algorithms for \sh with respect to the parameters such as treewidth \& number of colors, size of vertex cover, neighborhood diversity number, distance to threshold graph. Also we bound chromatic number by these parameters.

The \SH for a graph require only less number of colors and also the colored vertices dominate all the remaining vertices. In most of the graphs \sh can give better results than other coloring scheme. So that we can use the \SH in the applications which use minimum dominating set and conflict$-$free colouring.

==> diameter.tex <==
%The distance of two distinct vertices $u$ and $v$, denoted by $d(u, v)$, is the length of a shortest path connecting $u$ and $v$.


\begin{definition}

The diameter of $G$, denoted by diam(G), is defined as $diam(G)=\max{d(u, v)|u,v \in V(G)}$, where $d(u, v)$ is the distance of two distinct vertices $u$ and $v$.

\end{definition}


\begin{theorem}
The number of colors required to \SH coloring problem is W[2]-hard on general graphs of diameter 2.
\end{theorem}

\begin{proof}
The chromatic number of a \sh of a graph is bounded by the minimum dominating set of that graph. Since the diameter of this graph is two, vertices in dominating set are of distance at most two. Therefore we can not repeat the colors of vertices in the dominating set. This implies that the chromatic number of a \sh of a graph is equal to the minimum dominating set of diameter 2. Dominating set of a graph of diameter 2 is known as W[2]-hard.\cite{diameter}.

\end{proof}




==> honeycomb.tex <==
\begin{definition}
\cite{honeycomb} A honeycomb network
can be built from hexagons in various ways. A honeycomb network of size one is a single hexagon,
denoted by $h(1)$. Honeycomb network of
size $2$ denoted $h(2)$, can be obtained by
adding six hexagons around the boundary
edges of $h(1)$. In general, honeycomb
network $h(n)$ can be obtained from $h(n–1)$ by adding a layer of hexagons around the
boundary edges of $h(n – 1)$.
\end{definition}
% Alternatively, the size d of HC(n) is determined as the number of hexagons between the center and boundary of HC(n) (inclusive) and the number of vertices and edges of HC(n) are $6n^2$ and $9n^2-3n$ respectively. 
For a honeycomb network $h(n)$, we refer the set of hexagons in the first layer (innermost layer) as $h_1$ and in general, the set of hexagons in the $i^{th}$ layer as $h_i$. Thus $h_1$ has one hexagon, $h_2$ has $6$ hexagons and so on.
\begin{figure}[h]
\centering
\includegraphics[scale=0.6]{honeyEven.pdf}
\caption{The \sh~using one color $h(even)$ and $h(1)$.}
\label{Figure: label_honeyEven}
\end{figure}


\begin{lemma}
$\chi_{ssc}(h(n)) = 1$ if $n=1$ or $n$ is even. Otherwise $\chi_{ssc}(h(n)) = 2$.
\end{lemma}

\begin{proof}

The graph $h(1)$ can be $1$-subset square colored by coloring any two vertices which are at distance $3$. For $h(n)$ where $n$ is even, 
we color all vertex in $h_2$ such that the colored vertices in $h_2$ are at distance $3$ which can dominate a vertices in $h_1$. Further we dominate all vertices from $h_3$ by coloring the vertices from $h_3$ which are opposite to the colored vertices in $h_2$, refer figure \ref{Figure: label_honeyEven}. We repeat the process till all the vertices in $h_n$ are dominated by the vertices either from $h_n$ or vertices from $h_{n-1}$. In this coloring we can observe that all colored vertices are at distance $3$, since $1$-subset square coloring exists.

Furthermore we can color $h(n)$, where $n$ is odd and $n \neq 1$ using $2$ colors. For this refer bottom of the figure  \ref{Figure: label_honeyOdd}(c). 
We can color graph $h(n-1)$ using one color, since $n-1$ is even.  Now we can try to dominate all vertices in $h_{n}$ by coloring vertices in $h_n$ such that they are opposite to the colored vertices in $h_{n-1}$. Then we need new color on $h_{n}$, where adjacent hexagons in $h(n)$ is colored by color one.

 
\noindent Now we show that $2$ colors are necessary for $h(n)$, where $n$ is odd and $n \neq 1$.

We consider a graph $h(3)$, and try to dominate all vertices by using one color. For this we can examine different way of dominating the vertices of $h_1$, as follows.

\begin{enumerate}
\item Two vertices from $h(1)$, they are opposite to each other, say $v_1$ and $v_2$.
\begin{enumerate}
\item Let $p_1, p_2, p_3, p_4$ are the vertices on $h_3$ such that each of these vertices are at distance $3$ from either $v_1$ or $v_2$. Without loss of generality we can assume that $p_1$ and $p_2$ are at distance $3$ from $v_1$. Also we can observe that $p_1$ and $p_2$ have only one common neighbor $u_1$, since they are at distance $2$. Now we can not dominate $p_1$ or $p_2$ by a neighbor of $p_1$ or $p_2$ vertex from $h_2$ because those neighbors and $v_1$ are at distance $2$. Therefore to dominate $p_1$ and $p_2$ by coloring one of them or the common neighbor of them.

If we color $p_1$ or $p_2$, Without loss of generality we assume that $p_1$ is colored, then $p_2$ can 
only dominate by a vertex from $h_3$, which is at distance $3$ from $p_1$. Now if we try to extend this coloring by coloring the vertex which are opposite to the colored vertex, then we need extra color for some vertices on $h_{3}$. See figure \ref{Figure: label_honeyOdd}(a).

If we color the common neighbor $u_1$ of $p_1$ and $p_2$ to dominate $p_1$ and $p_2$ then, we can color the vertices from $h_3$, which is at distance $3$ from $u$. Now to dominate the vertices from $h_2$ which are at distance $2$ from $u_1$ can not dominate by using color one. See top of the figure \ref{Figure: label_honeyOdd}(b).
\end{enumerate}

\item None of the vertices from $h(1)$.
\begin{enumerate}
\item We can color every fourth vertex from $h_2$ to dominate vertices from $h_1$, refer bottom of the figure \ref{Figure: label_honeyOdd}(b) or bottom of the figure \ref{Figure: label_honeyOdd}(c). The vertex on $h_2$ which is opposite to $u_2$ on $h_{3}$ is colored. Now we can either color $u_2$ or $N(u_2)$. We can not dominate some the vertices on $h_3$ by using color one by similar argument of 1.(a). 
\end{enumerate}

\item One vertex from $h(1)$, remaining from $h(2)$.
\begin{enumerate}
\item If we start to dominate undominated vertex of $h_1$ by vertices from $h_2$, then the vertex on $h_2$ which is opposite to the vetex $u_2$ on $h_{3}$ is colored. Therefore we can not dominate some the vertices on $h_3$ by using color one. Refer figure \ref{Figure: label_honeyOdd}(c) or bottom of figure \ref{Figure: label_honeyOdd}(b).

\end{enumerate}
\end{enumerate}

\end{proof}



\begin{figure}[htb]
\centering
\includegraphics[scale=0.6]{HoneycombOdd.pdf}
\caption{The \sh~using one color $h(odd)$.}
\label{Figure: label_honeyOdd}
\end{figure}





%\begin{definition}
%\cite{honeycomb} A honeycomb network
%can be built from hexagons in various ways. A honeycomb network of size one is a single hexagon, denoted by $h(1)$. Honeycomb network of size $2$ denoted $h(2)$, can be obtained by adding six hexagons around the boundary edges of $h(1)$. In general, honeycomb network $h(n)$ can be obtained from $h(n –1)$ by adding a layer of hexagons around the
%boundary edges of $h(n – 1)$.
% Alternatively, the size d of HC(n) is determined as the number of hexagons between the center and boundary of HC(n) (inclusive) and the number of vertices and edges of HC(n) are $6n^2$ and $9n^2-3n$ respectively. 
%\end{definition}
%For a honeycomb network $h(n)$, we refer the set of hexagons in the first layer (innermost layer) as $h_1$ and in general, the set of hexagons in the $i^{th}$ layer  as $h_i$. Thus $h_1$ has one hexagon, $h_2$ has $6$ hexagons and so on.
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.6]{honeyEven.pdf}
%\caption{\sh using one color $h(even)$ and $h(1)$}
%\label{Figure: label_honeyEven}
%\end{figure}


%\begin{lemma}
%$\chi_{ssc}(h(n)) = 1$ if $n=1$ or $n$ is even. Otherwise $\chi_{ssc}(h(n)) = 2$.
%\end{lemma}

%\begin{proof}

%The graph $h(1)$ can be $1$-subset square colored by coloring any two vertices which are at distance $3$. For $h(n)$ where $n$ is even, 
%we color all vertex in $h_2$ such that the colored vertices in $h_2$ are at distance $3$ which can dominate every vertex in $h_1$. Further we dominate all vertices from $h_3$ by coloring the vertices from $h_3$ which are opposite to the colored vetices in $h_2$, refer figure \ref{Figure: label_honeyEven}. We repeat the process till all the vertices in $h_n$ are dominated by the vertices either from $h_n$ or vertices from $h_{n-1}$. In this coloring we can observe that all colored vertices are at least distance $3$, since $1$-subset square coloring exists.

%Furthermore we can color $h(n)$, where $n$ is odd and $n \neq 1$ using two colors. For this
%refer figure  \ref{Figure: label_honeyOdd}(d). 
%We can color graph $h(n-1)$ using one color, since $n-1$ is even.  Now we can try to dominate all vertices in $h_{n}$ by coloring vertices in $h_n$ using color one which are opposite to the colored vetices in $h_{n-1}$. Then we need new color on $h_{n}$, where adjacent hexagons in $h(n)$ is colored by color one.

%\end{proof}

%\begin{enumerate}
%\item Two vertices from $h(1)$, they are opposite to each other.
%	\begin{enumerate}
%	\item There exist four vertices from the outer cycle of $h(3)$ with distance three refer figure \ref{Figure: label_honeyOdd}(b). W.l.o.g consider $p_1$ and $p_2$ from figure \ref{Figure: label_honeyOdd}(b), are at distance two from each other. If we color using first color other vertex can not dominate using a vertex from outer cycle of $h(2)$. Therefore we need to dominated by a vertex from outer cycle of $h(3)$. We use the first color on every end vertex of $P_3$ from the colored vertex. If we continue this we will end up with some vertices which needs one more color refer top of the figure \ref{Figure: label_honeyOdd}(b). 
%	\item If we start to dominate the vertices from $h(2)$ by coloring the vertices from outer cycle of $h(2)$. It form a zigzac path and end up with uncolored and undominated vertex, refer figure \ref{Figure: label_honeyOdd}(a).
%\end{enumerate}
%\item None of the vertices from $h(1)$
%\begin{enumerate}
%\item If we color every fourth vertex from  the outer cycle of $h(3)$, refer figure \ref{Figure: label_honeyOdd}(c). We will be left with some vertex on outer cycle of $h(2)$.
%\item If we color every fourth vertex in a zigzag path from $h(2)$, refer figure \ref{Figure: label_honeyOdd}(d) and (c). We will be left with some vertex on outer cycle of $h(3)$.
%\end{enumerate}
%\item One vertex from $h(1)$, remaining from $h(2)$.
%\begin{enumerate}
%\item If we start to dominate undominated vertex of $h(1)$ by vertices from $h(2)$. We will be left with some vertex on outer cycle of $h(3)$, refer figure \ref{Figure: label_honeyOdd}(e).
%\end{enumerate}
%\end{enumerate}




%\begin{figure}[htb]
%\centering
%\includegraphics[scale=0.6]{HoneycombOdd.pdf}
%\caption{\sh using one color $h(even)$ and $h(1)$}
%\label{Figure: label_honeyOdd}
%\end{figure}



==> more_result.tex <==
\subsection{More results}

\begin{observation}
\label{one}
 If a graph $G$ has at least one vertex with degree $n-1$, then  $\chi_{ssc}(G) =1$.
\end{observation}

For a vertex $v \in V(G)$, if $d(v)=n-1$, then we can color only $v$ and it is a valid subset square coloring. Thus graphs like complete graphs, wheel graph, flower graph, double wheel graph, etc. are $1$-subset square colorable. We further discuss some more graph classes which can be subset square colored using a constant number of colors.

%In other words, if a graphs have cardinality of minimum dominating set is one, then $\chi_{ssc}(G)$ is also one. 

%Path graph is $1$-subset square coloring. We can reuse the color for every third vertex from the colored vertex in the path.
%Similar to the \sh of path, we can color a cycle with $3n$ vertices using one color, but we will be left with one$\backslash$ two vertices such that it neighbor are dominated (by using one color) in the cycles with $3n + 1$ or $3n + 2$ vertices. Therefore we need one more color to dominate undominated such vertices. So that cycle on $3n + 1$ or $3n + 2$ vertices have chromatic number is 2. The $\chi_{ssc}(G)$ needed for some other graph classes are given in the table \ref{tab:title},

\begin{lemma}
If $G$ is a path on n vertices then $\chi_{ssc}(G) = 1$.
\end{lemma}
\begin{proof}
%Any path on $n$ vertices requires exactly one color to be \shar colored. We give a constructive proof of this. 
Consider a path $P_n$ such that it has $3k$ or $3k + 2$ vertices where $k \geq 1$. We can color every third vertex beginning from the second vertex from one of the end vertices of the path. For path of length $3k+1$, we can color the first vertex using color 1 and every third vertex using the same color and so on. This ensures that every vertex is dominated by exactly one colored neighbor in its closed neighborhood.

\qed
\end{proof}



\begin{lemma}
If $G$ is a cycle on $3n$ vertices then $\chi_{ssc}(G) = 1$. Further, if $G$ is a cycle on $3n + 1$ or $3n + 2$ vertices then $\chi_{ssc}(G) = 2$.
\end{lemma}
\begin{proof}
For a cycle on $3n$ vertices, we color every third vertex and hence get a \sh using $1$ color. For cycles on $3n+1$ and $3n+2$ vertices, we use color $1$ to color every third vertex beginning from a vertex, say $v_1$, and finally use color $2$ to color the last vertex that appears in this sequence. 


%Furthermore, we note that one color is not sufficient for cycles on $3n + 1$ or $3n + 2$ vertices. Consider a cycle on $3n+1$ vertices. To \shar color this cycle using one color, we start by coloring vertex $v_1$ and assign the same color to every third vertex. We observe that the vertex $v_n$ is also assigned the same color as $v_1$, which does not \shar color vertices $v_1$ and $v_n$. Therefore, to avoid this conflict, we color vertex $v_n$ using a new color. Now consider a cycle on $3n+2$ vertices. We color the vertices using one color, as it was done for cycles on $3n+1$ vertices. We observe that vertices $v_1$ and $v_{n-1}$ of the cycle on $3n+2$ vertices are colored using the same color. So, to dominate vertex $v_n$, we assign it a new color. Therefore, for cycles on $3n+1$ and $3n+2$ vertices, we have $\chi_{S1H}(G) = 2$.
\qed
\end{proof}



%\noindent
%Now we study the nature of \sh coloring with resepect to threshold graphs.
%
%\begin{definition}
%\cite{golumbic} A graph is a threshold graph if it can constructed from the empty graph by repeatedly adding either an isolated vertex or a dominating vertex.
%\end{definition}
%
%
%\begin{lemma}
%If $G$ is a threshold graph then $\chi_{S1H}(G) = 1$.
%\end{lemma}
%
%\begin{proof}
%If isolated vertices are present, color them using the same color. By coloring the last introduced dominating vertex $v$, we can subset square color $G$ 
%\end{proof}




%\begin{definition}
%\cite{honeycomb} A honeycomb network
%can be built from hexagons in various ways. A honeycomb network of size one is a single hexagon, denoted by $h(1)$. Honeycomb network of size $2$ denoted $h(2)$, can be obtained by adding six hexagons around the boundary edges of $h(1)$. In general, honeycomb network $h(n)$ can be obtained from $h(n –1)$ by adding a layer of hexagons around the
%boundary edges of $h(n – 1)$.
% Alternatively, the size d of HC(n) is determined as the number of hexagons between the center and boundary of HC(n) (inclusive) and the number of vertices and edges of HC(n) are $6n^2$ and $9n^2-3n$ respectively. 
%\end{definition}
%For a honeycomb network $h(n)$, we refer the set of hexagons in the first layer (innermost layer) as $h_1$ and in general, the set of hexagons in the $i^{th}$ layer  as $h_i$. Thus $h_1$ has one hexagon, $h_2$ has $6$ hexagons and so on.
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.6]{honeyEven.pdf}
%\caption{\sh using one color $h(even)$ and $h(1)$}
%\label{Figure: label_honeyEven}
%\end{figure}


%\begin{lemma}
%$\chi_{ssc}(h(n)) = 1$ if $n=1$ or $n$ is even. Otherwise $\chi_{ssc}(h(n)) = 2$.
%\end{lemma}

%\begin{proof}

%The graph $h(1)$ can be $1$-subset square colored by coloring any two vertices which are at distance $3$. For $h(n)$ where $n$ is even, 
%we color all vertex in $h_2$ such that the colored vertices in $h_2$ are at distance $3$ which can dominate every vertex in $h_1$. Further we dominate all vertices from $h_3$ by coloring the vertices from $h_3$ which are opposite to the colored vetices in $h_2$, refer figure \ref{Figure: label_honeyEven}. We repeat the process till all the vertices in $h_n$ are dominated by the vertices either from $h_n$ or vertices from $h_{n-1}$. In this coloring we can observe that all colored vertices are at least distance $3$, since $1$-subset square coloring exists.

%Furthermore we can color $h(n)$, where $n$ is odd and $n \neq 1$ using two colors. For this
%refer figure  \ref{Figure: label_honeyOdd}(d). 
%We can color graph $h(n-1)$ using one color, since $n-1$ is even.  Now we can try to dominate all vertices in $h_{n}$ by coloring vertices in $h_n$ using color one which are opposite to the colored vetices in $h_{n-1}$. Then we need new color on $h_{n}$, where adjacent hexagons in $h(n)$ is colored by color one.

%\end{proof}

%\begin{enumerate}
%\item Two vertices from $h(1)$, they are opposite to each other.
%	\begin{enumerate}
%	\item There exist four vertices from the outer cycle of $h(3)$ with distance three refer figure \ref{Figure: label_honeyOdd}(b). W.l.o.g consider $p_1$ and $p_2$ from figure \ref{Figure: label_honeyOdd}(b), are at distance two from each other. If we color using first color other vertex can not dominate using a vertex from outer cycle of $h(2)$. Therefore we need to dominated by a vertex from outer cycle of $h(3)$. We use the first color on every end vertex of $P_3$ from the colored vertex. If we continue this we will end up with some vertices which needs one more color refer top of the figure \ref{Figure: label_honeyOdd}(b). 
%	\item If we start to dominate the vertices from $h(2)$ by coloring the vertices from outer cycle of $h(2)$. It form a zigzac path and end up with uncolored and undominated vertex, refer figure \ref{Figure: label_honeyOdd}(a).
%\end{enumerate}
%\item None of the vertices from $h(1)$
%\begin{enumerate}
%\item If we color every fourth vertex from  the outer cycle of $h(3)$, refer figure \ref{Figure: label_honeyOdd}(c). We will be left with some vertex on outer cycle of $h(2)$.
%\item If we color every fourth vertex in a zigzag path from $h(2)$, refer figure \ref{Figure: label_honeyOdd}(d) and (c). We will be left with some vertex on outer cycle of $h(3)$.
%\end{enumerate}
%\item One vertex from $h(1)$, remaining from $h(2)$.
%\begin{enumerate}
%\item If we start to dominate undominated vertex of $h(1)$ by vertices from $h(2)$. We will be left with some vertex on outer cycle of $h(3)$, refer figure \ref{Figure: label_honeyOdd}(e).
%\end{enumerate}
%\end{enumerate}




%\begin{figure}[htb]
%\centering
%\includegraphics[scale=0.6]{HoneycombOdd.pdf}
%\caption{\sh using one color $h(even)$ and $h(1)$}
%\label{Figure: label_honeyOdd}
%\end{figure}



%\input{honeycomb.tex}

==> mw.tex <==

We start by showing the connection between $\chi_{ssc}(G)$ and the modular width of the graph. We first define the modular width of a graph.
The modular width of graph $G$ is computed by virtue of four operations, namely creation of isolated vertex, disjoint union, complete join and substitution. More precisely, the modular width of $G$ equals the maximum number of operands used by any occurrence of  substitution operation. These four operations that are involved in modular decomposition of graph $G$ are described in \cite{modularwidth}. For the sake of completeness, we mention the four operations here.

\begin{definition}\label{mod_def} \cite{modularwidth} Algebraic operations involved to compute modular width of graph $G$.
\begin{itemize}
\item Create an isolated vertex;
\item The disjoint union of two graphs, i.e., the \textit{disjoint union} of two graph $G_1$ and $G_2$, denoted by $G_1 \otimes G_2$, is the graph with vertex set $V(G_1)\cup V(G_2)$ and edge set $E(G_1)\cup E(G_2)$;
\item The complete join of two graphs, i.e., the \textit{complete join} of two graphs $G_1$ and $G_2$, denoted by $G_1\oplus G_2$, is the graph with vertex set $V(G_1)\cup V(G_2)$ and edge set $E(G_1)\cup E(G_2)\cup \{ \{v, u\}: v\in V(G_1)$ and $u\in V(G_2)\}$.
\item The substitution operation with respect to some graph $G$ with vertices $v_1,\dots,v_n$, i.e., for graphs $G_1,\dots,G_n$ the substitution of the vertices of $G$ by the graphs $G_1,\dots,G_n$, denoted by $G(G_1,\dots,G_n)$, is the graph with vertex set $\underset{1 \leq i \leq n}\cup V(G_i)$ and edge set $\underset{1 \leq i \leq n} \cup E(G_i)\cup \{\{u, v\}:u \in V(G_i)$ and $v \in V(G_j)$, $v_i,v_j \in E(G)$ and $i\neq j\}$. Hence, $G(G_1,\dots,G_n)$ is obtained from $G$ by substituting every vertex $v_i \in V(G)$ with the graph $G_i$ and adding all edges between the vertices of a graph $G_i$ and the vertices of a graph $G_j$ whenever $\{v_i, v_j\} \in E(G)$.
\end{itemize}
\end{definition}

\begin{definition} \cite{modularwidth} Let $A$ be an algebraic expression that uses only the four operation as mentioned in Definition \ref{mod_def}. We define the width of $A$ as the maximum number of operands used by any occurrence of the substitution operation in $A$. Modular width of graph G, denoted as $w(G)$, is the least integer $m$ such that $G$ can be obtained from such an algebraic expression of width at most $m$.
\end{definition}
Cographs are the graphs that can be constructed from operations$-$creation of an isolated vertex, disjoint union of two graphs and  complete join of two graphs. By definition, the modular width of cographs is two \cite{coudert2019fully}.\\
Now we state our result. 
\begin{lemma}
\label{mww}
The maximum number of colours required to subset square colour a graph $G$ equals the modular width of $G$, that is, $\chi_{ssc}(G)\leq w(G)$.
\end{lemma}
\begin{proof}
Now we discuss the maximum number of colours required to subset square colour $G$ while we perform those operations. 
On introducing an isolated vertex, we colour it by using one colour. 
To dominate the vertices created as a result of disjoint union of two graphs, we can use maximum number of colours that were used in subset square colouring each subgraphs in the disjoint union operation. 
%The complete join operation involves introducing edges between the two sets of vertices on which we intend to perform a complete join. Edges are introduced between every pair of vertices of the two sets of vertices, in addition to the existing edges. By using exactly two colours and colouring one vertex in each partition, we subset square colour all vertices introduced thus far.
Now we consider the complete join operation on the subgraph $G_c$. Let $G_c= G_{c1} \otimes G_{c2}$. If a vertex $v$ in $V(G_{ci})$, $i=\{1, 2\}$ has degree $|G_i(V)|-1$, then $\chi_{ssc}(G_c)=1$. Otherwise we can colour an arbitrary vertex $v$ from each $G_{c1}$ and $G_{c2}$ using two distinct colours. Therefore the  value of $\chi_{ssc}$ is $ \leq 2$. 
Finally, we examine the substitution operation. We colour an arbitrary vertex $v$ in each $G_i$ using distinct colours. %Now for every vertex in $G_i$, the presence of coloured neighbour in $G_i$, a vertex may possibly be adjacent to another coloured vertex in $G_j$
Now for every vertex in $G_i$ may possibly be adjacent to another coloured vertex in $G_j$. Therefore the value of $\chi_{ssc}$ can be at most $w$.  
\end{proof}
%\qed

\noindent A Graph with modularwidth two are exactly the cograph \cite{coudert2019fully}. Now the result follows. 

\begin{corollary}
\label{cogra}
If $G$ is a cograph, then $\chi_{ssc}(G) \leq 2$.
\end{corollary}

In this subsection, we prove that there is an FPT algorithm. %solving this problem on the graphs of bounded modular width. 

\begin{theorem}\label{FPTmw}
The \SH~is FPT when parameterized by modular width.
\end{theorem}

The modular-width of a graph can also define based on its (unique) modular decomposition tree, and can be computed in linear time $O(n+ m)$ for graphs with $n$ vertices and $m$ edges. 

\begin{proof}
We use a bottom-up approach on the modular decomposition tree to solve \SH.

In this, the isolated vertex in the subgraph corresponds to a leaf node. Therefore the optimum number of colours used on the subgraph is one.
 

%the subgraph corresponds to leaves, which is created by the operation $O_1$. The optimum number of colours used on the subgraph is one.
%To dominate the isolated vertices in the subgraph corresponds to leaf nodes

Now, we consider other operations on combining two modules to form a larger module. If $G$ be the subgraph corresponds to a node, such that $G_d= G_{d1} \otimes G_{d2}$. The optimum number of colours used on $G_d$ is $max\{$optimum number of colours used on$(G_{d1})$, optimum number of colours used on$(G_{d2})\}$.

%maximum number of colours used in any of the two graphs. 


Next, we consider a subgraph $G_c$ corresponding to a node such that $G_c= G_{c1}\oplus G_{c2}$. If a vertex $v$ in $V(G_{ci})$, $i=\{1, 2\}$ has degree $G_i(V)-1$, then the optimum number of colours used on this node is $1$. Otherwise we colour one arbitrary vertex from each graph. Therefore the optimum number of colours used in this node is either $1$ or $2$.

%then $\chi_{ssc}(G_c)=1$. Otherwise we can colour an arbitrary vertex from $G_{c1}$ and $G_{c2}$ using two distinct colours.Therefore the value of $\chi_{ssc}$ of this node is either $1$or $2$.
%If the minimum dominating set of $G_1$ or $G_2$ is $1$ then the optimum number of colours used on this node is$1$. Otherwise we colour one arbitrary vertex from each graph.Therefore the optimum number of colours used in this node is either $1$ or $2$.

Now we consider the substitution operation with respect to $G$. In this operation we replace each vertex $v_i \in V(G)$ with the graph $G_i$ for $1 \leq i \leq w$. Therefore the vertices are in one-to-one correspondence with $G_i$. We try to colour the vertices in $G$ by bruteforce using $q$ colours.
%The graph $G_s$ can be colour by bruteforce, i.e, we can try all possible colouring on $G$ using $q$ colours, $q^w$. 

Let $G'= G(G_1,\dots,G_w)$. If we try to extend the colouring of $G$ to $G'$, we can colour an arbitrary vertex in $G_i$ if $v_i$ is coloured in $G$. If a vertex $v_i \in G$ does not have a coloured vertex in $N(v_i) \in G$ then to dominate vertices in $G_i$ we need to colour the vertices in $G_i$. 

Let $v'$ and $u'$ be the vertices in $G_i$, where colour of $u'$ in $G_i =$ colour of $v_i$ in $G$. We can restrict the number of colours that can be used for $v' \in G_i$ depending on its dominating set size of $G_i$. Since the number of $G_i$ is always limited by modular-width, we can calculate this in $2^{w(G)}$.

Let $q'$ be the number of colours that are used in $N(N(v))$ where $v \in G$. For all $G_i$, if the dominating set size of $G_i \leq q'$ then only \sh~exist on this node.

%Therefore, if the optimum number of colours is grater than $q'$, then only -\sh~exist on this node.

%We cannot assume much about the structure of the metagraph, but since its size is bounded, we can look at all the options and try them individually. This time, the two reasonable options for each module is to either not include it at all – when the module is covered by an adjacent module, or include one single vertex from the module to either cover all adjacent modules, or the module itself as well, depending on its dominating set size. Since the number of modules is always limited by modular-width, we can calculate this in 2m.


%If a vertex is self dominated in $G_i$, then to dominate other vertices in $G_i$ we need to colour some other vertices in $G_i$.



%in the node corresponding to the substitution if the optimum number of colours $q$ used in the subtree is grater than $q'$, then only -\sh~exist on this node.

%Therefore the optimum number of colours used on this node can be find in $q^{w}$, $q \leq w$.

It follows that the \SH~is FPT when parameterized by modular width.




==> mwFPT.tex <==
\subsection{Parameterized by modular width} \label{mwBondFPT}

We start by showing the connection between $\chi_{ssc}(G)$ and the modular width of the graph. 
For this we consider the modular decomposition tree of $G$.
%We can represent $G$ as an algebraic expression consisting of the following operations:

%\begin{definition} \cite{modularwidth} Let A be an algebraic expression that uses only the four operations as mentioned above. We define the width of A as the maximum number of operands used by any occurrence of the substitution operation in A. The modular width of a graph $G$, denoted $w(G)$, is the least integer $w$ such that $G$ can be obtained from such an algebraic expression of width at most $w$. Furthermore, an algebraic expression of width $w(G)$ can be constructed in linear time.
%\end{definition}

\begin{definition}\cite{modwidh}
Given a graph $G = (V,E)$, $M \subseteq V$ is called a module if $M$
is homogeneous with respect to any vertex $x \in V \setminus M$ (i.e. $M \subseteq N(x)$ or $M \cap N(x)= \phi$).
\end{definition}

A module $M$ is a strong module if it does not overlap with any other module. The inclusion tree of the strong modules of $G$, called the \textit{modular decomposition tree}, entirely represents the graph if the representative graph of each strong module is attached to each of its nodes. In modular decomposition tree, each node is created by one of the following operation.
\begin{itemize}
\item Create an isolated vertex ($O_1$).
\item The disjoint union of two graphs ($O_2$), i.e., the \textit{disjoint union} of two graphs $G_1$ and $G_2$, denoted by $G_1 \otimes G_2$, is the graph with vertex set $V(G_1)\cup V(G_2)$ and edge set $E(G_1)\cup E(G_2)$.
\item The complete join of two graphs ($O_3$), i.e., the \textit{complete join} of two graphs $G_1$ and $G_2$, denoted by $G_1\oplus G_2$, is the graph with vertex set $V(G_1)\cup V(G_2)$ and edge set $E(G_1)\cup E(G_2)\cup \{ \{v, w\}: v\in V(G_1)$ and $w\in V(G_2)\}$.
\item The substitution operation ($O_4$) with respect to some graph $G$ with vertices $v_1,\dots,v_n$, i.e., for graphs $G_1,\dots,G_n$ the substitution of the vertices of $G$ by the graphs $G_1,\dots,G_n$, denoted by $G(G_1,\dots,G_n)$, is the graph with vertex set $\underset{1 \leq i \leq n}\cup V(G_i)$ and edge set $\underset{1 \leq i \leq n} \cup E(G_i)\cup \{\{u, v\}:u \in V(G_i)$ and $v \in V(G_j)$, $v_i,v_j \in E(G)$ and $i\neq j\}$. Hence, $G(G_1,\dots,G_n)$ is obtained from $G$ by substituting every vertex $v_i \in V(G)$ with the graph $G_i$ and adding all edges between the vertices of a graph $G_i$ and the vertices of a graph $G_j$ whenever $\{v_i, v_j\} \in E(G)$.
\end{itemize}


The \textit{modular width} of $G$ is the maximum degree of the modular decomposition tree of $G$. The subgraphs $G_1, G_2, etc.$ defined in the above operations corresponds to the child nodes of the node corresponding to $G$. We now discuss, how to bound the value of $\chi_{ssc}$ in a subgraph $G$ which corresponds to a node in the modular decomposition tree.

\begin{lemma}
The maximum number of colours required to \sh~colour $G$ equals the modular width of the graph, that is, $\chi_{ssc}(G)\leq w(G)$.
\end{lemma}
\begin{proof}
We show how to subset square color a subgraph of $G$ corresponding to a node in the modular decomposition tree using at most $w$ colors.

To dominate the isolated vertices in the subgraph corresponds to leaf nodes, we color the vertices in the subgraph corresponding to leaves by using one color.

To dominate the vertices in the subgraph created as a result of disjoint union of two graphs, we can use maximum number of colors that were used in subset square coloring each subgraphs in the disjoint union operation. Therefore we can bound the value of $\chi_{ssc}$ on the corresponding node. 


Now we consider the node corresponding to a complete join operation on the subgraph $G_c$. Let $G_c= G_{c1} \otimes G_{c2}$. 
If a vertex $v$ in $V(G_{ci})$, $i=\{1, 2\}$ has degree $G_i(V)-1$, then $\chi_{ssc}(G_c)=1$. Otherwise 
We can color an arbitrary vertex from $G_{c1}$ and $G_{c2}$ using two distinct colors. Therefore the  value of $\chi_{ssc}$ of this node is $ \leq 2$. 
 

%To dominate the vertices in the subgraph created as a result of the complete join operation by using at most two colors. We can color arbitrary vertex from each two graphs which a one vertex in each graph, we subset square color all vertices introduced thus far. 

Finally, we examine the node corresponding to a graph created by the substitution operation. We color an arbitrary vertex $v$ in each $G_i$ using distinct colors. Apart from the presence of coloured neighbour(s) in $G_i$, a vertex may possibly be adjacent to another coloured vertex in $G_j$. Therefore the value of $\chi_{ssc}$ of node can be at most $w$. 

%We colour one vertex in each $G_i$. Besides the presence of coloured neighbour(s) in $G_i$, a vertex may possibly be adjacent to another coloured vertex in $G_j$. To \shar colour $G$, we would then require the number of operands in this operation.


%Therefore to subset square color $G$, we require at most $w$ colors.% the number of operands in this operation.
\end{proof}

Now we prove that there is an FPT algorithm solving this
problem on the graphs of bounded modular width. 
\begin{theorem}\label{FPTmw}
The \SH~is FPT when parameterized by modular width.
\end{theorem}

\begin{proof}

We use a bottom-up approach on the modular decomposition tree to solve \SH.

In this, the isolated vertex in the subgraph corresponds to a leaf node. Therefore the optimum number of colors used on the subgraph is one.
 

%the subgraph corresponds to leaves, which is created by the operation $O_1$. The optimum number of colors used on the subgraph is one.
%To dominate the isolated vertices in the subgraph corresponds to leaf nodes

Now, we consider other operations on combining two modules to form a larger module. If $G$ be the subgraph corresponds to a node, such that $G_d= G_{d1} \otimes G_{d2}$. The optimum number of colors used on $G_d$ is $max\{$optimum number of colors used on$(G_{d1})$, optimum number of colors used on$(G_{d2})\}$.

%maximum number of colors used in any of the two graphs. 


Next, we consider a subgraph $G_c$ corresponding to a node such that $G_c= G_{c1}\oplus G_{c2}$. If a vertex $v$ in $V(G_{ci})$, $i=\{1, 2\}$ has degree $G_i(V)-1$, then the optimum number of colors used on this node is $1$. Otherwise we color one arbitrary vertex from each graph. Therefore the optimum number of colors used in this node is either $1$ or $2$.

%then $\chi_{ssc}(G_c)=1$. Otherwise we can color an arbitrary vertex from $G_{c1}$ and $G_{c2}$ using two distinct colors.Therefore the value of $\chi_{ssc}$ of this node is either $1$or $2$.
%If the minimum dominating set of $G_1$ or $G_2$ is $1$ then the optimum number of colors used on this node is$1$. Otherwise we color one arbitrary vertex from each graph.Therefore the optimum number of colors used in this node is either $1$ or $2$.

Now we consider the substitution operation with respect to $G$. In this operation we replace each vertex $v_i \in V(G)$ with the graph $G_i$ for $1 \leq i \leq w$. Therefore the vertices are in one-to-one correspondence with $G_i$. We try to color the vertices in $G$ by bruteforce using $q$ colors.
%The graph $G_s$ can be color by bruteforce, i.e, we can try all possible coloring on $G$ using $q$ colors, $q^w$. 

Let $G'= G(G_1,\dots,G_w)$. If we try to extend the coloring of $G$ to $G'$, we can color an arbitrary vertex in $G_i$ if $v_i$ is colored in $G$. If a vertex $v_i \in G$ does not have a colored vertex in $N(v_i) \in G$ then to dominate vertices in $G_i$ we need to color the vertices in $G_i$. If $v$  vertex in $G_i$ we can restrict the number of colors that can be used for $v \in G_i$. Let $q'$ be the number of colors that are used in $N(N(v))$.


%If a vertex is self dominated in $G_i$, then to dominate other vertices in $G_i$ we need to color some other vertices in $G_i$.



Let $v$ be the vertex in $G_i$ we can restrict the number of colors that can be used for $v \in G_i$. Let $q'$ be the number of colors that are used in $N(N(v))$. 

Therefore, if the optimum number of colors is grater than $q'$, then only -\sh~exist on this node.

%in the node corresponding to the substitution if the optimum number of colors $q$ used in the subtree is grater than $q'$, then only -\sh~exist on this node.

%Therefore the optimum number of colors used on this node can be find in $q^{w}$, $q \leq w$.

It follows that the \SH~is FPT when parameterized by modular width.
\qed


\end{proof}




==> preliminaries.tex <==


\noindent\textbf{X3C (Exact cover by 3-sets) :} Instance A finite set $X$ with $|X|=3n$ and a collection $S$ of $3-$element subsets of $X$ with $|S| = m$.\\
\textbf{Question:} Does $S$ contain an exact cover for $X$ , i.e., a subcollection $S' \subseteq S$ such that every element of $X$ occurs in exactly one member of $S'?$



==> q_Nopoly.tex <==
The proof is very similar to that of Theorem 2. We give a reduction from
the X3C problem. Similar to the previous proof, we construct

\begin{theorem}
The $q$-\sh~parameterized by vertex cover size does not have a polynomial kernel, unless $NP \subseteq coNP/poly$, for $q \geq 3$.
\end{theorem}



We use the same technique \textit{OR}-cross-composition defined in the previous section. In this reduction also we consider $t$ instances of the \textsc{Clique} problem, $X_1,X_2, \cdots ,X_t$ of the clique under the polynomial equivalence relation $\textit{R}$ such that if the number of vertices of each $X_i$ is $n$ and asks for a $k$ sized clique. 





\noindent We modify the definition of the special vertex as follows.\\
\noindent \textbf{Special vertex :} If a vertex $v$ is a special vertex, then $N(v)$ contain $q+1$ single degree vertices. We denote the special vertex by two circles with the same centre and different radius.\\


\begin{observation}
\label{dum2}
For any $q$-\sh~$C$ of $G$,if a vertex $v$ in $G$ is a special vertex, then $C(v) \neq c_0$. 
\end{observation}

We start to create an instance of $G$ for $q$-\sh{}. Let's start the graph construction by adding a set of $q$ vertices, $Q= \{Q_1, Q_2, \cdots Q_q\}$. We add an edges between all vertices . Let's consider all the vertices in set $Q$ are special vertices in $G$. Without loss of generality, we assume that $C(Q_1)=$colour $q_1$, $C(Q_2)=$ colour $q_2$ and so on.

%Continue the construction of $G$ 
%
%We proceed with the construction of $G$ with a set of vertices and edges.

Now we add a set of vertices $\{ p_{i,j}|i \in [k], j \in [n] \}$. %Let $P$ be the set of all $p_{i,j}$ vertices. 
The set of all $p_{i,j}$ vertices is called grid vertices of $G$. Similar to the graph constructed in $2$-\sh{}reduction, these vertices are also used to select the vertices that correspond to a clique in one of the input instances.

%\noindent We will create number of different gadgets in this construction of $G$, and we will add those gadgets to grid vertices and special vertices $R$ and $B$. 

In order to complete the construction, We modify all the gadgets that used in the proof of $2$-\sh~parameterized by vertex cover size kernel.  In this modification we make sure that $s^{i,j}_{j,j'}$ can not dominated by itself and for all $i \in [k], j \in [n]$, $C(p_{i,j})=\{$red, $c_0\}$. 

For every $i \in [k]$,  we add a path gadget $\mathcal{P}1_i$ with three vertices $r'_i, r_i,$ and $ r''_i$. In every $\mathcal{P}1_i$, there exist edges $(r'_i, r_i)$ and $(r_i, r''_i)$, where $r_i$ is a special vertex. These vertices form a path $P_3$ in the path gadget. Connect path gadget$\mathcal{P}1_i$ to the set of vertices in $Q$, by adding edges between $r_i$ and $\{Q_3, Q_4 \cdots Q_q\}$. See Figure \ref{path}. Also path gadget$\mathcal{P}1_i$ connect to grid vertices through $r_i$ by adding edges $(r_i, p_{i,j})$, for all $j\in [n]$.
Similiarly for every $j \in [n]$, we use a similar path gadget, $\mathcal{P}2_j$ with  three $w_j$, $w'_j$ and $w''_j$. In every $\mathcal{P}2_j$, there exist edges $(w_j, w'_j)$ and $(w'_j, w''_j)$, where $w'_j$ is a special vertex.  In addition to that add edges between $w_j$ and $\{Q_3, Q_4 \cdots Q_q\}$. Connect all $w''_j$ with all vertices in $Q$ except $Q_2$. Also connect the vertices $w$ and $Q_1$. See Figure \ref{tree}. Moreover, we connect $\mathcal{P}2_j$ with grid vertices by adding edges $(w_j,p_{i,j})$, for all $i \in [k]$. Connect path gadget$\mathcal{P}2_j$ to the set of vertices in $Q$, by adding an edge between all $w_j$ and $w$


\begin{figure}[th]
	\begin{minipage}[b]{0.53\linewidth}
		\centering
		%\includegraphics[width=\textwidth]{orthogonal.pdf}}
		\includegraphics[width=4.5cm]{qpath.pdf}
		\caption{Path gadget $\mathcal{P}1_i$ connected with set of vertices in $Q$}
		\label{qpath}
	\end{minipage}
	\hspace{1cm}
	\begin{minipage}[b]{0.38\linewidth}
		\centering
		%\includegraphics[width=\textwidth]{edge_rect.pdf}
		\includegraphics[width=3.5cm]{qtree.pdf}
		\caption{Path gadget $\mathcal{P}2_j$ connected with set of vertices in $Q$}
		\label{qtree}
		
	\end{minipage}
\end{figure}

We continue the construction of $G$ by creating a \textit{connector gadget} $S^{i,i'}_{j,j'}$, for every $i, i' \in [k]$ and $j,j' \in [n]$, where $i < i'$ and $j < j'$. The connector gadget $S^{i,i'}_{j,j'}$ contains seven vertices $c_1, c_2 \cdots, c_6$, $s^{i,i'}_{j,j'}$, $q-1$ copies of $c_4, c_5$ and $c_6$. where all $q$ vertices $c_5$ are a special vertices. We add edges $(c_1, c_2), (c_2,c_3), (c_2,s^{i,i'}_{j,j'}), (c_3,c_5),$


\noindent$(c_3, s^{i,i'}_{j,j'}), (c^1_4,s^{i,i'}_{j,j'}), (c^1_4,c_1), (c^1_4, c_5)$ and $(c_5,c_6)$ in $S^{i,i'}_{j,j'}$. Add edges between all $q-1$ copies of $c^1_4$ with $s^{i,i'}_{j,j'}$ and $c_2$. Also add edges between $c^t_4$ and $c^t_5$, where $1 \leq t \leq q-1$. Add edges between all $q-1$ copies of $c^1_5$ and $c_2$. Also add edges between $c^t_6$ and $c^t_5$, where $1 \leq t \leq q-1$. Connect $S^{i,i'}_{j,j'}$ to the set of vertices in $Q$, by adding an edge between $c_1$ with all vertices in $Q$ except $Q_1$. Also first copy of $c_6$ connect with $q_1= R$, second copy of $c_6$ connect with $q_1 $ and $q_2$, third copy of $c_6$ connect with $q_1, q_2$ and $q_3$ and so on. See Figure \ref{qcon}.
The connector gadget connect with grid vertices through $c_1$ and $c_2$. Connect the vertices $c_1$ and $c_2$ in the connector gadget $S_{j,j'}^{i,i'}$ with $p_{i',t''}$ and $p_{i,t'}$ respectively, where $t'\in \{j,j'\}$ and $t''\in \{j,j'\}$.

\begin{figure}[th]
	\begin{minipage}[b]{0.53\linewidth}
		\centering
		%\includegraphics[width=\textwidth]{orthogonal.pdf}}
		\includegraphics[width=5cm]{qconnector.pdf}
		\caption{Connector gadget connected with set of vertices in $Q$}
		\label{qcon}
	\end{minipage}
	\hspace{.5cm}
	\begin{minipage}[b]{0.38\linewidth}
		\centering
	\includegraphics[width=5.5cm]{qhanging.pdf}
\caption{Hanging gadget connected with set of vertices in $Q$}
	\label{qhang}
	\end{minipage}
\end{figure}


Furthermore,  for all $i \in [k]$ we create a hanging gadget $\mathcal{H}_i$ with five vertices, $\{h_i, h'_i, h''_i, f_i, d_i\}$ and $q$ copies of the vertex $f_i= \{f^1_i, f^2_i \cdots f^q_i\}$  and $q$ copies of $d_i =\{d^1_i, d^2_i \cdots d^q_i\}$, where all $f^t_i$,$1 \leq t \leq q$ are special vertices in $\mathcal{H}_i$. 


The vertices $h_i, h'_i, h''_i, f^t_i$, where $1 \leq t \leq q$ are form cycles in $\mathcal{H}_i$. The vertices $f^t_i$, where $1 \leq t \leq q$ are special vertices in $\mathcal{H}_i$. Other vertices $d^t_i$ are connect with $f^t_i$, where $1 \leq t \leq q$. Hanging gadget $\mathcal{H}_i$ connected to $Q$, by adding edges between $d^t_i$ and $Q_t \in Q$, where $1 \leq t \leq q$. See Figure \ref{qhang}. In addition to that every $h_i$ connect with grid vertices $p_{i,j}$, for all $j\in [n]$.

\begin{lemma}
\label{qhanging}
For any $q$-\sh~$C$ of $G$, $C(h_i), C(h'_i)$ and $C(h''_i)$ will be $c_0$ for all values of $i \in [k]$.
\end{lemma}
\begin{proof}
%In a hanging gardget $\mathcal{H}_i$ contains two special verices $f_i$ and $f'_i$. Therefore these vertices need to be coloured (follows from observation \ref{dum}).

Since the vertices $h_i, h'_i$ and $h''_i$ are at a distance at most $2$ from at least one of the special vertices $f^t_i$, where $1 \leq t \leq q$ we cannot colour them.
\qed
\end{proof}

We can observe from the Lemma \ref{qhanging} that we cannot dominate the vertex $h_i$ by colouring the vertex from $N[h_i] \in \mathcal{H}_i$ and all other vertices in $\mathcal{H}_i$ are dominated by at least one of the special vertices $f^t_i$, where $1 \leq t \leq q$.

Furthermore, we add a \textit{selector gadget} $\mathcal{Y}$ with set of vertices $Y=\{y_l|1 \leq l \leq t\}$ and four vertices $z_1, \cdots, z_4$, where $z_2$ is a special vertex. For all $l \in [t]$, we connect $y_l$ with $z_1$ and $z_2$. The vertex $z_4$ connected to $z_1$.  Additionaly add an edge between $z_2$ and $z_3$. This $\mathcal{Y}$ shows which of the instances has a clique of size $k$. Connect the hanging gadet to the set of vertices in $Q$, by adding edges between $(z_3,Q_2)$ and $(z_2,Q_t|3 \leq t\leq q)$. In addition to these edges $(z_4,Q_t|1 \leq t\leq q)$. See Figure \ref{qhg}.



	  
\begin{figure}[tbh]
 \centering
\includegraphics[width=6.5cm]{qselector.pdf}
\label{qhg}
\caption{Selector gadget}
\end{figure}

Now we have completed the construction of graph $G$. The following lemmas will help to prove the correctness.

\begin{lemma}
\label{qoneRed}
For any $q$-\sh~$C$ of $G$, there exist distinct $j_1, \cdots j_k$ such that $C(p_{i,j_i})=$ red and every other grid vertices $p$, $C(p)=c_0$.  
\end{lemma}
\begin{proof}	
From Lemma \ref{qhanging}, we need a vertex in $N(h_i) \cap \{p_{i,j}| 1 \leq j \leq n \}$, to dominate each $h_i$ for all $i \in [k]$. Let $p_{i,j_i}$ be the vertex, for each $i \in [k]$, there exist at most one $j \in [n]$ such that $C(p_{i,j})=$ red. Since there exists an edge between $r_i$ and  $p_{i,j}$, for all $j \in [n]$, every grid vertices are dominated by the special vertex $r_i$ from $\mathcal{P}1_i$. 

For each $j \in [n]$, there is exactly one $i \in [k]$ such that $C(p_{i,j})=$ red. Consider the vertex special $w'_j$ in $\mathcal{P}2_j$, $N(N(w'_j))$ contains $Q_t|t\neq 2 and 1 \leq t \leq q$, therefore $C(w'_j)=$ blue. Now we can observe that exactly one vertex in $p_{i,j}$ for all $i \in [k]$ get red colour and there exists an edge $(w_j, p_{i,j})$, for all $i \in [k]$. Therefore all $j_i$ are distinct.
\qed
\end{proof}


\begin{lemma}
\label{qoneBlue}
For any $q$-\sh~$C$ of $G$, there exists exactly one vertex in $Y$, $y_l \in \{y_i|i \in [t]\}$ such that $C(y_l)=$ blue and every other vertex $y \in Y$ where $y \neq y_l$, $C(y)= c_0$.   
\end{lemma}
\begin{proof}	
In $\mathcal{Y}$, every vetex other than $z_1$ are dominated by the special vertex $z_2$. Since the vertex $z_4$ is connected to special vertex $z_2$ and all $Q_t|2 \leq t \leq q$, we can not dominate $z_1$ using $z_1$ or $z_4$. Only the vertex $\{y_l| l \in [t]\}$ can dominate the vertex $z_1$, but every $\{y_l|1 \leq l \leq t\}$ is at distance two apart from each other. Therefore only one vertex from $\{y_l| l \in [t]\}$ can dominate the vertex $z_1$. 

The special vertex $z_2$ is at most distance two apart from $Q_t|2 \leq t \leq q$. Therefore $C(z_2)=$ red and one vertex $C(y_l)=$ blue, where $y_l \in \{y_i|i \in [t]\}$. Also every other vertices $y \in Y$ where $y \neq y_l$, $C(y)= c_0$. 
\qed
\end{proof}

\noindent Now, we claim the main theorem as follows.
%
%\begin{theorem}
%\label{theorem1}
%If there exists an instance $X_l$ that has a \textsc{Clique }of size $k$ if and only if $G$ can be $2$-subset square coloured.
%\end{theorem} 


\begin{theorem}
\label{theorem2}
The graph $G$ is $q$-subset square colorable if and only if there exists $l \in [t]$ such that instance $X_l$ has a \textsc{Clique} of size $k$.
\end{theorem} 
\begin{proof}
 
Let assume, there exists a yes instance $X_l$ such that, it has a \textsc{Clique }of size $k$. We select $v_{j_1}, \cdots v_{j_k} \in [n]$ such that these vertices form a clique in $X_l$. Now we colour the graph $G$ as follows.

\begin{enumerate}
\item Colour the vertices in $Q$, such that $C(Q_1)= q_1$,$C(Q_2)=q_2$ and so on.

\item Let $C(f^t_i)=q_t$(by observation \ref{dum} and there exist edges $(f^t_i,d^t_i)$ in $G$).

\item Since $w''_j$ is connected to $R$, $C(w'_j)=$ blue.

\item $C(c_5)=$ blue (by observation \ref{dum} and $N(N(c_5))$ contain $Q_t|t\neq 2 and 1 \leq t \leq q$).

\item Since $z_3$ is connected to $B$ and $z_2$ is connected to $Q_t|3 \leq t \leq q$, $C(z_2)=$ red.

\item Since $r'_i$ is connected to $R$ and $r_i$ connected to $Q_t|3 \leq t \leq q$, $C(r_i)=$ blue.
 
\item Let $C(y_l)=$ blue, ($y_l$ dominates the vertex $z_1$, $N(z_2)$ contain $Q_t|3 \leq t \leq q$).
  
\item Let $C(p_{i,j_i})=$ red for all $i \in [k]$ (dominates the vertex $h_i$) and other vertices are coloured with $c_0$ (dominated by the vertex $r_i$) . 

\item If $p_{i,t'}$ and $p_{i',t''}= c_0$ where $t'\in \{j,j'\}$ and $t''\in \{j,j'\}$, then $C(c_3)=$ red.

\item If $p_{i,t'} = c_0$ and $p_{i',t''}=$ red where $t'\in \{j,j'\}$ and $t''\in \{j,j'\}$, then $C(c_3)=$ red 

\item If $p_{i,t'} =$ red and $p_{i',t''}= c_0$ where $t'\in \{j,j'\}$ and $t''\in \{j,j'\}$, then $C(c_4)=$ red.


\end{enumerate}


%----
The vertex $s^{i,i'}_{j,j'}$ verifies that if we select vertices $v_j$ and $v_j'$ to be part of the \textsc{Clique}, then no instance $X_l$ where $\{v_{j},v_{j'}\} \in E(X_l)$ can be selected as the yes instance. The connector gadget helps to do this.

If  $p_{i',t''} = p_{i,t'}=$ red, where $t'\in \{j,j'\}$ and $t''\in \{j,j'\}$,then undominated vertex $s^{i,i'}_{j,j'}$ can not dominated by using any of the vertex $c_3, c_2$ or $c^t_4$ because $N[c_3, c_2$ or $c^t_4]$ contain colours $\{q_1, q_2 \cdots q_q\}$.
Since the vertex $s^{i,i'}_{j,j'}$ is distance two from $c_5$ and $p_{i,t'}$, we can not colour the vertex $s^{i,i'}_{j,j'}$ using any colour from $\{q_1, q_2 \cdots q_q\}$. Therefore edge $(s^{i,i'}_{j,j'}, y_l)$ exists to dominate the vertex $s^{i,i'}_{j,j'}$.

For every $l \in [t]$, $i, i' \in [k]$, and $j, j' \in [n]$, add an edge $(s^{i,i'}_{j,j'}, y_l)$ if and only if ${v_j,v_{j'}} \in E(X_l)$. If ${v_j,v_{j'}} \not \in E(X_l)$ then the following lemma holds.

\begin{lemma}
\label{CaseStudy}
If one of the $p_{i,t'}$ or $p_{i',t''}$ where $t'\in \{j,j'\}$ and $t''\in \{j,j'\}$ is red or none of them is red, then there exist a \sh~$C$, such that $C(c_3)$ or $C(c_4) =$red. 
\end{lemma}
\begin{proof}	
Since the vertex $c_6$ is connected to the vertex $R$ and $c_5$ is a special vertex. Therefore we need to colour $c_5$ using blue. We can continue this proof by case analysis. We need to dominate the vertices $s^{i,i'}_{j,j'}$ and $c_2$ in $S^{i,i'}_{j,j'}$, all other vertices are dominated by themselves or by their neighbours.

\begin{enumerate}
\item If $p_{i,t'}$ and $p_{i',t''}=$ colour $c_0$, then to dominate the vertices $s^{i,i'}_{j,j'}$ and $c_2$ in $S^{i,i'}_{j,j'}$, we can colour the vertex $c_3$. Since $C(c_5)=$ blue and $(c_5, c_3)$ exists. we can colour $c_3$ using red. 

\item If $p_{i',t''} =$ red and $p_{i,t'}=$ colour $c_0$, then to dominate the vertices $s^{i,i'}_{j,j'}$ and $c_2$, we can colour $c_3$ using red.

\item If $p_{i,t'} =$ red and $p_{i',t''}=$ colour $c_0$, then to dominate the vertex $s^{i,i'}_{j,j'}$ we can colour $c_4$ using red. The coloured vertex $p_{i,t'}$ will dominate the vertex $c_2$. 

%\item If $p'_i = p_i =$red,then undominated vertex $s^{i,i'}_{j,j'}$ can not colour using red. Since the vertex $s^{i,i'}_{j,j'}$ is distance two from $c_5$, we can not colour the vertex $s^{i,i'}_{j,j'}$ using blue also. Therefore edge $(s^{i,i'}_{j,j'}, y_l)$ exists for to satisfy $2$-\sh.
\end{enumerate}
\end{proof}
%-----


 


Now it is easy to verify that every vertex $v$ and $N[v]$ in $G$ satisfies the $2$-\sh~constrains. Therefore this colouring in $G$ is a valid $q$-\sh. See Figure \ref{Pmain}.
 
Now we can prove, if $G$ can be $2$-subset square colored, then there exists $l \in [t]$ such that instance $X_l$ has a \textsc{Clique} of size $k$.

From Lemma \ref{qoneBlue}, we know that, there exists $y \in Y$, with $C(y)=$ blue. We can pick $l$ such that $\{y_l|l \in [t]\}$ By lemma \ref{oneRed}, take distinct $j_1 \cdots j_k \in [n]$ such that $C(p_{i, j_i}) =$ red. We will show that instance $X_l$ has a
\textsc{Clique} of size $k$, by proving that vertices $v_{j_1} \cdots v_{j_k} \in [n]$ form a \textsc{Clique} in $X_l$.
Assume that this is not true. Then there exist $i, i' \in [k]$ such that $v_{j_i}$ and $v_{j'_i}$ are not connected by an edge in $X_l$. This will leads to a contradiction. Let consider connector gadget $S^{i,i'}_{j_i,j'_ i}$, the vertices $p_{i',t''}$ and $p_{i,t'}$ are colored with red, where $t'\in \{j,j'\}$ and $t''\in \{j,j'\}$. 



Since the vertex $s^{i,i'}_{j,j'}$ is distance two from $c^1_5$ and $p_{i,t'}$, we can not colour the vertex $s^{i,i'}_{j,j'}$ using red or blue. Therefore edge $(s^{i,i'}_{j,j'}, y_l)$ exists for to dominate  $s^{i,i'}_{j,j'}$. It now follows that $(s^{i,i'}_{j,j'}, y_l) \not \in G$, which contradicts that $C$ is a \sh~of $G$. 

\qed
\end{proof}
To prove the lower bound,
it remains to bound the size of a vertex cover in $G$. Since vertices in $Y$ form an independent set in $G$, it follows that $V (G) \backslash (Y=\{y_l| 1 \leq l \leq t\})$ is a vertex cover of $G$. 

Number of grid vertices $G$ is at most $n \times k$ and for every pair of vertices in grid vertices has a connector gadget $S^{i,i'}_{j,j'}$. Therefore 
total number of vertices in connector gadgets is at most $7 \times (n^2 \times k^2)+ q \times 3$. Therefore $|V (G) \backslash Y| = O(n^2 \cdot k^2)$.

We can conclude that the \SH~problem parameterized by the size of vertex cover does not have a polynomial kernel for $q \geq 3$ using \textit{OR}- cross composition from \textsc{Clique}.


==> twin_cover.tex <==
\begin{definition}
\cite{twin} For a graph $G(V,E)$ a subset $X$ of vertices is twin cover if for every edge $e=uv \in E(G)$ either
 \begin{enumerate}
\item $u \in X$ or $v \in X$, or 
\item $u$ and $v$ are true twins. 
\end{enumerate} 
Two vertices $u$ and $v$ are true twin if all other vertices are adjacent to both $u,v$ or none.
\end{definition}

\begin{theorem}
The \SH parameterized by the size of twin cover is FPT.
\end{theorem}
Let $G(V,E)$ be the graph and $X \subset V$ be the set of vertices such that $G[V-X]$ have either cliques or independent vertices as per the definition of twin cover. 
If $q \geq k$, then by Lemma(define) it is trivally true that a subset square coloring exists. Therefore, we assume that $q<k$.

Consider all possible ${(q+1)}^k$ coloring of $X$ using $\{c_0,c_1, \dots c_q}$. Here coloring a vertex by $c_0$ corresponts to a vertex not being colored. 


 We say a coloring $\chi_G$ of $V$ \emph{extends} $\chi$ if  $\chi_G$ restricted to $X$ is $\chi$. Our algorithm tries to extend each of the colorings to a valid subset square coloring using $q$ colors of $G$ as follows. 
Let $I = V\setminus X$. Let $W \subseteq I$ be the set of vertices that are not dominated by $\chi$. Note that vertices in $V-X$ induces disjoint union of cliques and independent set. Also, from construction of twin cover if $v \in X$ adjacent to a clique vertex in $V-X$ then it will be adjacent to all other vertices of the clique. So, we can replace each clique to single vertex which make the set $V-X$ as independent set. Now the reduced graph is similar to vertex cover and we can proceed in same way.


 Thus $U$ has at most $2^k$ vertices which we can color in $\mathcal{O}(q^{2^k})$ or $\mathcal{O}(k^{2^k})$  time as $q \leq k$. Hence the running time of the algorithm is $\mathcal{O}(k^{2^k})$.
